Field-theoretic functional renormalization group formalism for non-Fermi liquids and its application to the antiferromagnetic quantum critical metal in two dimensions

To capture the universal low-energy physics of metals within effective field theories, one has to generalize the usual notion of scale invariance and renormalizable field theory due to the presence of intrinsic scales (Fermi momenta). In this paper, we develop a field-theoretic functional renormalization group formalism for full low-energy effective field theories of non-Fermi liquids that include all gapless modes around the Fermi surface. The formalism is applied to the non-Fermi liquid that arises at the antiferromagnetic quantum critical point in two space dimensions. In the space of coupling functions, an interacting fixed point arises at a point with momentum-independent couplings and vanishing nesting angle. In theories deformed with non-zero nesting angles, coupling functions acquire universal momentum profiles controlled by the bare nesting angles at low energies before flowing to superconducting states in the low-energy limit. The superconducting instability is unavoidable because lukewarm electrons that are coherent enough to be susceptible to pairing end up being subject to a renormalized attractive interaction with its minimum strength set by the nesting angle. Despite the inevitable superconducting instability, theories with small bare nesting angles and bare four-fermion couplings that are repulsive or weakly attractive must pass through the region with slow RG flow due to the proximity to the non-Fermi liquid fixed point. The bottleneck region controls the scaling behaviours of the normal state and the quasi-universal pathway from the non-Fermi liquid to superconductivity. In the limit that the nesting angle is small, the non-Fermi liquid scaling dictates the physics over a large window of energy scale above the superconducting transition temperature.

==> 4beta.tex <==

\subsubsection{Full Beta function for $\lambda^{1551}$}

\begin{enumerate}

\item $ p=-k, l \neq q -2k$:
\begin{equation}
\begin{aligned}
 \frac{\partial}{\partial\ell}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}  &= 
%\\ =& 
%-k\frac{\partial}{\partial k}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}} - l \frac{\partial}{\partial l}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}  \\& 
- \left( 1 + 3(z-1) +  {\eta}^{(\psi)}_{k+l} 
 + {\eta}^{(\psi)}_{-k-l} +  {\eta}^{(\psi)}_{k} +  {\eta}^{(\psi)}_{-k} \right) {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}
\\ &
 - \frac{1}{\pi}\int\dd \rho(q)\sum_{\beta, \alpha = 1}^{N_c} 
 \left\lbrace \frac{1}{4} {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right. \\ &
 +  \left.
 \left[ \frac{1}{2} {\lambda}^{\spmqty{4 & 8 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}}
 % \right. \right. \\ & \left. \left.\rule{0em}{2em} 
-\frac{1}{N_f}\mathsf{T}_{\sigma_2 \alpha ; \sigma_1 \beta}\mathsf{D}( k + l; q) \right] \left[ \frac{1}{2} {\lambda}^{\spmqty{4 & 8 \\ 1 & 5};\spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}}  -\frac{1}{N_f}\mathsf{T}_{\sigma_3 \alpha ; \sigma_4 \beta}\mathsf{D}(q; k)  \right] \right\rbrace.
\end{aligned}
\label{eq:betalambda1PP}
\end{equation}

\item $ p=k+l$:
\begin{equation}
\begin{aligned}
 \frac{\partial}{\partial\ell}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}} & 
  = 
  %-k\frac{\partial}{\partial k}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}  
  %- l \frac{\partial}{\partial l}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}  \\
 % &
   - \left( 1 + 3(z-1) + 2 {\eta}^{(\psi)}_{k+l} + 2 {\eta}^{(\psi)}_{k} \right) {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}
\\ & - \frac{1}{\pi}\int\dd \rho(q)\sum_{\beta, \alpha = 1}^{N_c} \left\lbrace \frac{1}{4} {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} \right. \\
& \left.
+ \left[ \frac{1}{2} {\lambda}^{\spmqty{1 & 8 \\ 4 & 5};\spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}} 
\rule{0em}{2em} -\frac{1}{N_f}\mathsf{T}_{\beta \sigma_1 ; \sigma_3 \alpha}\mathsf{D}(q; k + l) \right] \left[ \frac{1}{2} {\lambda}^{\spmqty{4 & 5 \\ 1 & 8};\spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}}  -\frac{1}{N_f}\mathsf{T}_{\alpha \sigma_2 ; \sigma_4 \beta}\mathsf{D}(q; k)  \right] \right\rbrace.
\end{aligned}
\label{eq:betalambda1PH}
\end{equation}

\item $l = 2p = -2k$:
%\begin{equation}
%\begin{aligned}
%& \frac{\dd \lambda^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k & -k}}}{\dd \log\mu} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + \frac{\partial\log Z^{(\psi)}(-k)}{\partial\log\mu} + \frac{\partial\log Z^{(\psi)}(k)}{\partial\log\mu} \right)\lambda^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k & -k}}
%\\ & -\frac{1}{\pi N_f}\int\frac{\dd  q }{2\pi}\left\lbrace \frac{1}{\mu/2 + c\abs{q} + \abs{2v_{k-q}k}} \left[ \frac{g_{k,k-q}^2}{V_{F,k-q}}\left( \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 \sigma_3}}_{\spmqty{-k+ q & k- q \\ k & -k}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k+ q & k- q \\ k & -k}} \right) \right. \right.
%\\ & \left. -\frac{g_{k,k-q}g_{k-q,k}}{V_{F,k-q}}\left( \sum_{\alpha=1}^{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{-k+ q & k- q \\ k & -k}}\delta_{\sigma_1 \sigma_3} - \frac{1}{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k+ q & k \\ k & -k+q}} \right)\right]
%\\ & + \frac{1}{\mu/2 + c\abs{q} + \abs{2 v_{k+q}k}} \left[ \frac{g_{k+q,k}^2}{V_{F,k+q}}\left( \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{-k & k \\ k+ q & -k-q}} -\frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k+ q & -k-q}} \right) -\frac{g_{k+q,k}g_{k,k+q}}{V_{F,k+q}}\left(\sum_{\alpha=1}^{N_c} \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{-k & k+ q \\ k+ q & -k}}\delta_{\sigma_2 \sigma_4} \right. \right.
%\\ & \left. \left. \left. -\frac{1}{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k+ q \\ k+ q & -k}} \right) \right] \right\rbrace
%\\ & +\frac{2\mu}{\pi N_f^2}\left[ 4\left( 1 + \frac{1}{N_c^2} \right)\delta_{\sigma_1\sigma_4}\delta_{\sigma_2 \sigma_3} - \frac{8}{N_c}\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} \right]\int\frac{\dd q}{2\pi}\frac{g_{q,-k}^2 g_{k,q}^2}{ V_{F,q}} \frac{1}{c(\abs{ q - k} + \abs{v_ q  q + v_{k} k})+ \mu/2}
%\\ & \times\frac{1}{c(\abs{ q + k} + \abs{v_ q  q - v_{k}k}) + \mu/2} -\frac{\mu}{\pi N_f^2}\left[4 \left( N_c - \frac{2}{N_c} \right)\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}+\frac{4}{N_c^2}\delta_{\sigma_1 \sigma_4} \delta_{\sigma_2 \sigma_3}\right]
%\\ & \times\int \frac{\dd q}{2\pi}\frac{g^2_{q, k}g^2_{-k, q}}{V_{F, q}}\frac{1}{(c(|q-k| + |v_{q}q+v_{k}k|) +\mu/2 ) (c(|q+k| + |v_{q}q-v_{k}k|)+\mu/2 )} 
%\\ & + \frac{1}{2 \mu} \int \frac{\dd q}{2\pi} \frac{1}{2\pi V_{F,k+q}}\sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{-k & k \\ k+ q & -k-q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{k+ q & -k- q \\ k & -k}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{-k & k \\ k+ q & -k-q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{k+ q & -k- q \\ k & -k}} \right).
%\end{aligned}
%\end{equation}
\begin{equation}
\begin{aligned}
&  \frac{\partial}{\partial\ell} 
\lambda^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k & -k}} = 
- \left( 1 + 3(z-1) + 2 {\eta}^{(\psi)}_{k} + 2 {\eta}^{(\psi)}_{-k} \right) 
\lambda^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k & -k}}\\ & 
- \frac{1}{\pi N_f}\int\dd \rho(q)
\left\lbrace  
\mathsf{D}(-k; q)
%\frac{g_{-k,q}g_{q,-k}}{\pi N_f}\frac{1}{\mu + c(\abs{q+k} + \abs{v_{q} q - v_{k}k})}
\left[ \left( \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right)  -\left( \sum_{\alpha=1}^{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}}\delta_{\sigma_1 \sigma_3} - \frac{1}{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & k \\ k & q}} \right)\right] \right. \\ 
& \left. +
\mathsf{D}(q; k)
%
%\frac{g_{q,k}g_{k,q}}{\pi N_f}\frac{1}{\mu + c(\abs{q-k} + \abs{v_{q} q + v_{k}k})} 
\left[ \left( \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{-k & k \\  q & -q}} -\frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\  q & -q}} \right) -\left(\sum_{\alpha=1}^{N_c} \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}}\delta_{\sigma_2 \sigma_4} 
 -\frac{1}{N_c}\lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}} \right) \right] \right\rbrace
\\ & - \frac{1}{\pi N_f^2} 
\left[ 4\left( 1 + \frac{1}{N_c^2} \right)\delta_{\sigma_1\sigma_4}\delta_{\sigma_2 \sigma_3} - \frac{8}{N_c}\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} \right]
\int\dd \rho(q)
\mathsf{D}(-k; q)
\mathsf{D}(q; k) \\
%
%\int\frac{\dd q}{2\pi}\frac{1}{ V_{F,q}} \frac{g_{q, k}g_{k,q}g_{q,-k}g_{-k, q}}{\mu + c(\abs{ q - k} + \abs{v_ q  q + v_{k} k})}
%\\ & \times\frac{1}{\mu + c(\abs{ q + k} + \abs{v_ q  q - v_{k}k})} 
%
& -\frac{1}{\pi N_f^2} 
\left[4 \left( N_c - \frac{2}{N_c} \right)\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}+\frac{4}{N_c^2}\delta_{\sigma_1 \sigma_4} \delta_{\sigma_2 \sigma_3}\right]
\int\dd \rho(q)
\mathsf{D}(k; q)
\mathsf{D}(q; -k)
%
%
%\\ & \times\int \frac{\dd q}{2\pi}\frac{1}{V_{F, q}}\frac{g_{q, k}g_{k,q}g_{q,-k}g_{-k, q}}{(\mu + c(|q-k| + |v_{q}q+v_{k}k|)) (\mu + c(|q+k| + |v_{q}q-v_{k}k|))} 
\\ & - \frac{1}{4\pi} \int\dd \rho(q)
%\int \frac{\dd q}{2\pi} \frac{1}{V_{F,q}}
\sum_{\alpha, \beta = 1}^{N_c}\left[\left(\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{-k & k \\  q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{-k & k \\  q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right)\right.
\\ & \left. - \left(\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} + \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} \right)\right].
\end{aligned}
\label{eq:PP&PH1}
\end{equation}




\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k & -k}} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + \frac{\partial\log Z^{(\psi)}(-k)}{\partial\log\mu} + \frac{\partial\log Z^{(\psi)}(k)}{\partial\log\mu} \right)\lambda^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\ k & -k}}
\\ & +\int\frac{\dd  q }{2\pi}\frac{1}{V_{F,q}}\left\lbrace -\frac{g_{-k,q}g_{q,-k}}{\pi N_f}\frac{1}{\mu + c(\abs{q+k} + \abs{v_{q} q - v_{k}k})} \left[ \left( \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right) \right. \right.
\\ & \left. -\left( \sum_{\alpha=1}^{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}}\delta_{\sigma_1 \sigma_3} - \frac{1}{N_c}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & k \\ k & q}} \right)\right]
\\ & -\frac{g_{q,k}g_{k,q}}{\pi N_f}\frac{1}{\mu + c(\abs{q-k} + \abs{v_{q} q + v_{k}k})} \left[ \left( \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{-k & k \\  q & -q}} -\frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k & k \\  q & -q}} \right) -\left(\sum_{\alpha=1}^{N_c} \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}}\delta_{\sigma_2 \sigma_4} \right. \right.
\\ & \left. \left. \left. -\frac{1}{N_c}\lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}} \right) \right] \right\rbrace
\\ & +\frac{\mu}{\pi N_f^2}\left[ 4\left( 1 + \frac{1}{N_c^2} \right)\delta_{\sigma_1\sigma_4}\delta_{\sigma_2 \sigma_3} - \frac{8}{N_c}\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} \right]\int\frac{\dd q}{2\pi}\frac{1}{ V_{F,q}} \frac{g_{q, k}g_{k,q}g_{q,-k}g_{-k, q}}{\mu + c(\abs{ q - k} + \abs{v_ q  q + v_{k} k})}
\\ & \times\frac{1}{\mu + c(\abs{ q + k} + \abs{v_ q  q - v_{k}k})} -\frac{\mu}{\pi N_f^2}\left[4 \left( N_c - \frac{2}{N_c} \right)\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}+\frac{4}{N_c^2}\delta_{\sigma_1 \sigma_4} \delta_{\sigma_2 \sigma_3}\right]
\\ & \times\int \frac{\dd q}{2\pi}\frac{1}{V_{F, q}}\frac{g_{q, k}g_{k,q}g_{q,-k}g_{-k, q}}{(\mu + c(|q-k| + |v_{q}q+v_{k}k|)) (\mu + c(|q+k| + |v_{q}q-v_{k}k|))} 
\\ & + \frac{1}{4\pi \mu} \int \frac{\dd q}{2\pi} \frac{1}{V_{F,q}}\sum_{\alpha, \beta = 1}^{N_c}\left[\left(\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{-k & k \\  q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{-k & k \\  q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right)\right.
\\ & \left. - \left(\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} + \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{-k &  q \\  q & -k}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} \right)\right].
\end{aligned}
\label{eq:PP&PH1}
\end{equation}

\item $k= p=l=0$:
Initially, by including all counter-term, we have:
\begin{equation*}
\begin{aligned}
& \frac{\dd \lambda^{\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}}{\dd \log\mu} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + 2\frac{\partial\log Z^{(\psi)}(0)}{\partial\log\mu} \right) \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & - \frac{1}{\pi N_f}\int\frac{\dd  q }{2\pi}\frac{1}{\mu + c(1+v_q)\abs{q}}\frac{g_{0,q}g_{q,0}}{V_{F,q}}\left\lbrace \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} +  \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{0 & 0 \\  q & -q}}  \right.
\\ &  -\frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\  q & -q}} - \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\delta_{\sigma_2 \sigma_4} + \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}}\delta_{\sigma_1 \sigma_3} \right) + \frac{1}{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}} \right.
\\ & \left. \left. + \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & 0 \\ 0 & q}} \right) \right\rbrace + \frac{v_0}{2\pi c N_f}\left[ \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)\right.
\\ & \left. - \frac{1}{N_c} \left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\right) \right] + \left( 2 \text{li}_2\left(-\frac{1}{2}\right) + \pi^2 + \log^2(2) \right)\frac{v_0^2}{4 N_f^2 c}\left( \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} - N_c \delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} \right)
\\ & + \frac{1}{2 \mu} \int \frac{\dd q}{2\pi} \frac{1}{2\pi V_{F,q}}\sum_{\alpha, \beta = 1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\  q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\  q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} \right.
\\ & \left. - \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}} - \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}}\right).
\end{aligned}
\end{equation*}
The last term in this expression corresponds to the source term and represents a total subtraction of the quantum effective action. Since this term is a constant, not depending on any IR divergences, and we are limiting ourselves to a minimal subtraction scheme we drop this term. The final answer is then
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + 2\frac{\partial\log Z^{(\psi)}(0)}{\partial\log\mu} \right) \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & - \frac{1}{\pi N_f}\int\frac{\dd  q }{2\pi}\frac{1}{\mu + c(1+v_q)\abs{q}}\frac{g_{0,q}g_{q,0}}{V_{F,q}}\left\lbrace \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} +  \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{0 & 0 \\  q & -q}}  \right.
\\ &  -\frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\  q & -q}} - \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\delta_{\sigma_2 \sigma_4} + \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}}\delta_{\sigma_1 \sigma_3} \right) + \frac{1}{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}} \right.
\\ & \left. \left. + \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & 0 \\ 0 & q}} \right) \right\rbrace + \frac{v_0}{2\pi c N_f}\left[ \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)\right.
\\ & \left. - \frac{1}{N_c} \left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\right) \right]
\\ & + \frac{1}{2 \mu} \int \frac{\dd q}{2\pi} \frac{1}{2\pi V_{F,q}}\sum_{\alpha, \beta = 1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\  q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\  q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} \right.
\\ & \left. - \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}} - \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}}\right).
\end{aligned}
\end{equation}

\end{enumerate}

\subsubsection{Full Beta function for $\lambda^{4851}$}

\begin{enumerate}

\item $ p=-k, l \ne q - 2k$:
%\begin{equation}
%\begin{aligned}
%& \frac{\dd \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}}{\dd\log\mu} = 
%\\ & \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(k+l)}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(-k-l)}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(k)}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(-k)}{\partial\log\mu} \right)\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}
%\\ & - \frac{1}{\pi N_f}\int\frac{\dd  q }{2\pi}\left[ \frac{g_{k+l,k+l+q}^2}{V_{F,k+l+q}}\frac{1}{\mu/2 + c\abs{q} + \abs{2v_{k+l+q}(k+l)}} \left(\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l+ q & -k-l- q \\ k & -k}} - \frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l+ q & -k-l- q \\ k & -k}} \right)\right.
%\\ & \left. + \frac{g_{k+q,k}^2}{V_{F,k+q}}\frac{1}{\mu/2 + c\abs{q} + \abs{2v_{k+q}k}}\left(\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{k+l & -k-l \\ k+ q & -k-q}} - \frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k+ q & -k-q}} \right) \right]
%\\ & + \frac{1}{2 \mu} \int \frac{\dd q}{2\pi} \frac{1}{2\pi V_{F,k+q}}\sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\ k+ q & -k-q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{k+ q & -k- q \\ k & -k}} + \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\ k+ q & -k-q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{k+ q & -k- q \\ k & -k}} \right).
%\end{aligned}
%\end{equation}
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}} = 
\\ & \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(k+l)}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(-k-l)}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(k)}{\partial\log\mu} + \frac{1}{2}\frac{\partial\log Z^{(\psi)}(-k)}{\partial\log\mu} \right)\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}
\\ & + \int\frac{\dd  q }{2\pi}\frac{1}{V_{F,q}}\left\lbrace -\frac{1}{\pi N_f}\left[\frac{g_{k+l,q}g_{q,k+l}}{\mu + c\abs{q-k-l} + \abs{v_{q} q + v_{k+l}(k+l)}} \left(\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} - \frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right) \right. \right.
\\ &  \left. +\frac{g_{q,k}g_{k,q}}{\mu + c\abs{q-k} + \abs{v_{q} q + v_{k} k}}\left(\lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{k+l & -k-l \\  q & -q}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\  q & -q}} \right)\right]
\\ &\left. + \frac{1}{4\pi\mu}\sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right)\right\rbrace.
\end{aligned}
\end{equation}
In terms of the logarithmic length scale
\begin{equation}
\begin{aligned}
& \frac{\partial}{\partial \ell} {\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}} = -k\frac{\partial}{\partial k} {\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}-l\frac{\partial}{\partial l} {\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}
\\ & -\left( 1 + 3(z-1) +  {\eta}^{(\psi)}_{k+l} +  {\eta}^{(\psi)}_{-k-l} +  {\eta}^{(\psi)}_{k} +  {\eta}^{(\psi)}_{-k} \right) {\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k-l \\ k & -k}}
\\ & - \frac{1}{\pi}\int \dd \rho(q)\sum_{\beta, \alpha = 1}^{N_c} \left\lbrace -\frac{1}{2 N_f}\left[\mathsf{D}(q;k +l)\mathsf{T}_{\sigma_2 \alpha ; \sigma_1 \beta}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right. \right. 
\\ & \left. + \mathsf{D}(q;k)\mathsf{T}_{\sigma_3 \alpha ; \sigma_4 \beta}  {\lambda}^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}}\right]
\\ &\left. + \frac{1}{4}\left( {\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}} {\lambda}^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} +  {\lambda}^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{k+l & -k-l \\  q & -q}} {\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ k & -k}} \right)\right\rbrace.
\end{aligned}
\label{eq:betalambda2PP}
\end{equation}

\item $k= p=l=0$:
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + 2\frac{\partial\log Z^{(\psi)}(0)}{\partial\log\mu} \right) \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & +\frac{v_0}{4\pi N_f}\frac{\pi v_0 + 2c(1+v_0)\log(c(1+1/v_0))}{c^2(1+v_0)^2+v_0^2}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 5 \\ 1 & 8} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{4 & 5 \\ 1 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\right]
\\ & \frac{1}{\pi N_f} \int\dfrac{\dd  q }{2\pi}\frac{g_{q,0}g_{q,0}}{V_{F,q}} \frac{1}{\mu + c(1+v_q)\abs{q}}\left[ \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{0 & 0 \\  q & -q}}  - \frac{1}{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\  q & -q}} \right) \right]
\\ & + \frac{1}{2 \mu} \int \frac{\dd q}{2\pi} \frac{1}{2\pi V_{F,q}}\sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\  q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\  q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & - q \\ 0 & 0}} \right).
\end{aligned}
\end{equation}

\end{enumerate}

\subsubsection{Full Beta function for $\lambda^{4581}$}

\begin{enumerate}

\item $ p=k+l$:
%\begin{equation}
%\begin{aligned}
%& \frac{\dd \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}}{\dd\log\mu} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu}+ \frac{\partial\log Z^{(\psi)}(k+l)}{\partial\log\mu} + \frac{\partial\log Z^{(\psi)}(k)}{\partial\log\mu} \right)\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}
%\\ & + \frac{1}{\pi N_f}\int\frac{\dd  q }{2\pi}\left[ \frac{g_{k+q,k}g_{k,k+q}}{V_{F,k+q}}\frac{1}{\mu/2 + c \abs{q} + \abs{2v_{k+q}k}}\left( \sum_{\alpha = 1}^{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{k+l & k+ q \\ k+ q & k+l}}\delta_{\sigma_2 \sigma_4} - \frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k+ q \\ k+ q & k+l}} \right) \right.
%\\ & \left. + \frac{g_{k+l+q,k+l}g_{k+l,k+l+q}}{V_{F,k+l+q}}\frac{1}{\mu/2 + c\abs{q}+\abs{2v_{k+l+q}(k + l)}}\left( \sum_{\alpha = 1}^{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{k+l+ q & k \\ k & k+l+q}}\delta_{\sigma_1 \sigma_3} - \frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l+ q & k \\ k & k+l+q}} \right) \right]
%\end{aligned}
%\end{equation}
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu}+ \frac{\partial\log Z^{(\psi)}(k+l)}{\partial\log\mu} + \frac{\partial\log Z^{(\psi)}(k)}{\partial\log\mu} \right)\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}
\\ & + \frac{1}{\pi N_f}\int\frac{\dd  q }{2\pi}\frac{1}{V_{F,q}}\left[ \frac{g_{q,k}g_{k,q}}{\mu + c \abs{q-k} + \abs{v_{q} q + v_{k} k}}\left( \sum_{\alpha = 1}^{N_c}\lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}}\delta_{\sigma_2 \sigma_4} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}} \right) \right.
\\ &  + \frac{g_{q,k+l}g_{k+l,q}}{\mu + c\abs{q-k-l}+\abs{v_{q} q + v_{k+l}(k + l)}}\left( \sum_{\alpha = 1}^{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}}\delta_{\sigma_1 \sigma_3} - \frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & k \\ k & q}} \right)
\\ & \left. - \frac{1}{4\pi \mu} \sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} \right) \right].
\end{aligned}
\end{equation}
In terms of the logarithmic length scale
\begin{equation}
\begin{aligned}
\frac{\partial}{\partial \ell} {\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}} = & -k\frac{\partial}{\partial k} {\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}-l\frac{\partial}{\partial l} {\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & -k \\ k & k+l}}
\\ & -\left( 1 + 3(z-1) + 2 {\eta}^{(\psi)}_{k+l} + 2 {\eta}^{(\psi)}_{k} \right) {\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{k+l & k \\ k & k+l}}
\\ & - \frac{1}{\pi}\int \dd \rho(q)\sum_{\beta, \alpha = 1}^{N_c} \left\lbrace \frac{1}{2 N_f}\left[\mathsf{D}(q;k)\mathsf{T}_{\alpha \sigma_2 ; \sigma_4 \beta}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}} \right. \right.
\\ & \left. + \mathsf{D}(q;k+l)\mathsf{T}_{\beta \sigma_1 ; \sigma_3 \alpha}  {\lambda}^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}}\right]
\\ &\left. - \frac{1}{4}\sum_{\alpha, \beta = 1}^{N_c}\left( {\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}} {\lambda}^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} +  {\lambda}^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{k+l &  q \\  q & k+l}} {\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & k \\ k & q}} \right)\right\rbrace.
\end{aligned}
\label{eq:betalambda3PH}
\end{equation}

\item $k= p=l=0$:
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + 2\frac{\partial\log Z^{(\psi)}(0)}{\partial\log\mu} \right) \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & + \frac{v_0}{4\pi N_f}\frac{\pi v_0 + 2c(1+v_0)\log(c(1+1/v_0))}{c^2(1+v_0)^2+v_0^2}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 4 & 8} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 8 \\ 1 & 5} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{4 & 8 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} \right]
\\ & +\frac{1}{\pi N_f} \int\dfrac{\dd  q }{2\pi}\frac{g_{0,q}g_{q,0}}{V_{F,q}}\frac{1}{\mu + c(1+v_q) \abs{q}}\left[ \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}}\delta_{\sigma_1 \sigma_3} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\delta_{\sigma_2 \sigma_4}  \right) \right. 
\\ & \left. -\frac{1}{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{ q & 0 \\ 0 & q}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}} \right) \right]
\\ & - \frac{1}{2 \mu} \int \frac{\dd q}{2\pi} \frac{1}{2\pi V_{F,q}}\sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 &  q \\  q & 0}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{ q & 0 \\ 0 & q}} \right)
\end{aligned}
\end{equation}

\end{enumerate}

\subsubsection{Full Beta function for $\lambda^{4554}$}

Only for $k= p=l=0$:

The full linear contribution to the beta function, in a total subtraction scheme is:
\begin{equation*}
\begin{aligned}
\frac{\dd \lambda^{\spmqty{4 & 5 \\ 4 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}}{\dd \log\mu} = & \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + 2\frac{\partial\log Z^{(\psi)}(0)}{\partial\log\mu} \right) \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & - \frac{v_0}{2\pi c(1+v_0) N_f}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} \right]
\\ & + \left( \frac{\pi^2}{4} + \log\left(\frac{27}{4}\right) \right)\frac{v_0^2}{2 N_f^2 c}\left( N_c\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} - \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} \right).
\end{aligned}
\end{equation*}
Only including IR divergences in the source term, as expected in a minimal subtraction scheme, we drop the last term, obtaining:
\begin{equation}
\begin{aligned}
\frac{\dd \lambda^{\spmqty{4 & 5 \\ 4 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}}{\dd \log\mu} = & \left( 1 + 3\frac{\partial \log Z_{\tau}}{\partial\log\mu} + 2\frac{\partial\log Z^{(\psi)}(0)}{\partial\log\mu} \right) \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & - \frac{v_0}{2\pi c(1+v_0) N_f}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} \right].
\end{aligned}
\end{equation}







==> etc.tex <==

\section{ETC}
\subsubsection{Delta Function Approximation}


In our second attempt to obtain any approximated solutions to Eqs. \eqref{eq:betaallwaves} we  argue that $\lambda$ behaves like a delta function in this regime, i.e., from Eq. \eqref{eq:physicalchange}, we write
\begin{equation}
\overline{\lambda}^{\mathrm{I}}_{k}\delta(k-p) = e^{\ell}\tilde{\lambda}^{\mathrm{I}}_{K}\delta(K-P)
\label{eq:deltafa}
\end{equation}
(here we can see the role of $e^{\ell}$ is to counter the $e^{-\ell}$ scale factor from $\delta(K-P)$.) Additionally, $\mathsf{R}$ also behaves like a delta function, in rescaled momentum:
\begin{equation}
\begin{aligned}
\frac{2\mathsf{T}_{\sigma_4 \sigma_1; \sigma_3 \sigma_2}}{N_f}\mathsf{R}( K, P) \approx & \frac{2\mathsf{T}_{\sigma_4 \sigma_1; \sigma_3 \sigma_2}}{N_f}\Lambda_f z (\hat{g}_{K,P})^2\frac{2(\Lambda_f + 2 \hat{v}_K c \abs{P})}{c}\frac{\Lambda_f}{(\Lambda_f + 2 \hat{v}_K c\abs{K})^2}\delta(K-P) \spmqty{0 & 1 \\ 1 & 0}
\\ = & 2\pi\Lambda_f\frac{\Lambda_f}{\Lambda_f + 2 v_K c\abs{K}}w^{(\mathsf{R})}_{{\sigma_4 \sigma_1; \sigma_3 \sigma_2}}(K,P)\delta(K-P)\spmqty{0 & 1 \\ 1 & 0}.
\end{aligned}
\label{eq:Rdelta}
\end{equation}
where
\begin{equation}
w^{(\mathsf{R})}_{{\sigma_4 \sigma_1; \sigma_3 \sigma_4}}(K,P) = \frac{2z(\hat{g}_{K,P})^2}{\pi c N_f}\mathsf{T}_{\sigma_4 \sigma_1; \sigma_3 \sigma_2}
\label{eq:weightR}
\end{equation}
is what we call the weight of the $\mathsf{R}$-term.
% Eq \eqref{eq:Rdelta} works as long as
%\begin{equation}
%\abs{\frac{\partial_K \hat{v}_{K}}{\hat{v}_{K}}}^{-1} \lesssim 2\frac{\Lambda_f + 2 v_K c \abs{K}}{c},
%\label{eq:adiabatichypothesis}
%\end{equation}
%i.e. the momentum scale over which $v$ at $K$ varies is less than the effective width of the function $\mathsf{R}$ (see Sec \ref{sec:adiabatic}.) Eq.\eqref{eq:adiabatichypothesis} needs to be proven in order for our approximation to be valid.
In terms of the $\tilde{r}$-function,
\begin{equation}
\begin{aligned}
\tilde{r}(\ell;K,P) = & 2\pi\Lambda_f\frac{\Lambda_f}{\Lambda_f + 2 \hat{v}_K c\abs{K}}w^{(\tilde{r})}(K,P)\delta(K-P),
\\ w^{(\tilde{r})}(K,P) = & \frac{z(\hat{g}_{K,P})^2}{\pi c}.
\end{aligned}
\end{equation}
In physical momentum $k, p$
\begin{equation}
\begin{aligned}
\tilde{r}(\ell;k, p) = & 2\pi\Lambda_f e^{-\ell} \frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}w^{(\tilde{r})}(k,p)\delta(k-p),
\\ w^{(\tilde{r})}(k,p) = & \frac{z(g_{k,p})^2}{\pi c}.
\end{aligned}
\end{equation}
so that Eq. \eqref{eq:betaallwaves} look like
%\begin{subequations}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{k} = & -\frac{1}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k, k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k,k})^2(N_c^2 -1)}{\pi c N_c N_f} \frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right)
%\\ & + \Lambda_f \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\left[\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right]^2 -\frac{4\Lambda_f}{N_f}\left(1-\frac{1}{N_c}\right) \frac{z(g_{k,k})^2}{c}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}},
%\label{eq:symsdelta}
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{k} = & -\frac{1}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k, k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right)
%\\ & \hspace{2cm}\times \left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}\right)
%\\ & + \Lambda_f \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\left[\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right]^2 + \frac{4\Lambda}{N_f}\left(1-\frac{1}{N_c}\right)\frac{z(g_{k,k})^2}{c}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}.
%\label{eq:symddelta}
%\end{aligned}
%\end{equation}
%\end{subequations}
%For the singlet channel:
%\begin{subequations}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{k} = & -\frac{1}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k, k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right)
%\\ & \hspace{2cm} \times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}\right)
%\\ & + \Lambda_f \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\left[\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right]^2 +\frac{4\Lambda_f}{N_f}\left(1+\frac{1}{N_c}\right) \frac{z(g_{k,k})^2}{c}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}},
%\label{eq:antisymsdelta}
%\end{aligned}
%\end{equation}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (\pm),(d)}_{k} = & -\frac{1}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (\pm),(d)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k, k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}\right)
%\\ & \hspace{2cm} \times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (\pm),(d)}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}\right)
%\\ & + \Lambda_f \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\left[\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right]^2 - \frac{4\Lambda_f}{N_f}\left(1+\frac{1}{N_c}\right)\frac{z(g_{k,k})^2}{c}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}.
%\label{eq:antisymddelta}
%\end{aligned}
%\end{equation}
%\end{subequations}
%In terms of Eq. \eqref{eq:betaallwaves},
\begin{equation}
\begin{aligned}
\frac{\dd }{\dd\ell}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k} = & -\frac{1}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k, k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}\right)
\\ & \hspace{2cm} \times\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}\right)
\\ & + \Lambda_f \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\left[\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}} \right]^2 + 1^{\spmqty{s \\ d}} \frac{4\Lambda_f}{N_f}\left(\frac{1}{N_c} \mp 1\right)\frac{z(g_{k,k})^2}{c}\frac{\Lambda_f}{\Lambda_f + 2 v_k c\abs{k}e^{\ell}}.
\label{eq:betaalldelta}
\end{aligned}
\end{equation}

We can discard the terms of order $g^4/c^2$ in the last equations. In limit $\abs{k} \ll \Lambda_f/(c v e^{\ell})$, the term $\Lambda_f/(\Lambda_f + 2 c v_k \abs{k}e^{\ell}) \sim 1$:
\begin{equation}
\begin{aligned}
\frac{\dd }{\dd\ell}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k} = & -\frac{1}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k, k})^2(N_c^2 -1)}{\pi c N_c N_f}\right)\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k} + \sqrt{2\pi}\Lambda_f \frac{(g_{k,k})^2(N_c^2 -1)}{\pi c N_c N_f}\right)
\\ & + 1^{\spmqty{s \\ d}} \frac{4\Lambda_f}{N_f}\left(\frac{1}{N_c} \mp 1\right)\frac{z(g_{k,k})^2}{c}.
\label{eq:betaalldeltalimit}
\end{aligned}
\end{equation}
The solution to this equation is
\begin{equation}
\begin{aligned}
\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k}(\ell) = & -\frac{2\Lambda_f (g_{k,k})^2 (N_c^2 - 1)}{c N_c N_f} 
\\ & - 4\pi\Lambda_f\sqrt{1^{\spmqty{s \\ d}}}\sqrt{\frac{z(\pm N_c - 1)(g_{k,k})^2}{c N_c N_f}}\tan\left[\sqrt{1^{\spmqty{s \\ d}}}\sqrt{\frac{z(\pm N_c - 1)(g_{k,k})^2}{c N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right)\right],
\end{aligned}
\label{eq:solregionI}
\end{equation}
where $\mathcal{C}_0$ is an integration constant depending on the boundary conditions on $\ell = 0$. The general equation for $\mathcal{C}_0$ is
\begin{equation}
\begin{aligned}
\mathcal{C}_0 =  & \frac{1}{4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f\sqrt{1^{\spmqty{s \\ d}}}}\sqrt{\frac{c N_c N_f}{z(\pm N_c - 1)(g_{k,k})^2}}
\\ & \hspace{1cm}\times\tan^{-1}\left[\frac{1}{4\pi\Lambda_f\sqrt{1^{\spmqty{s \\ d}}}}\sqrt{\frac{c N_c N_f}{z(\pm N_c - 1)(g_{k,k})^2}}\left( \overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{k}(0) + \frac{2\Lambda_f (g_{k,k})^2 (N_c^2 - 1)}{c N_c N_f}\right)\right]
\end{aligned}
\end{equation}

 The critical value of $\lambda$ is attained at at a value $\ell^{(1)}_k$ where $\lambda(\ell^{(1)}_k)$ diverges. Notice that for the $d$-wave $1^{\spmqty{s \\ d}} = -1$, and the triplet channel 
\begin{equation}
\overline{\lambda}^{\mathrm{I}; (+),(d)}_{k}(\ell) = -\frac{2\Lambda_f (g_{k,k})^2(N_c^2 - 1)}{c N_c N_f} + 4\pi\Lambda_f\sqrt{\frac{z(g_{k,k})^2(N_c - 1)}{c N_c N_f}}\tanh\left[\sqrt{\frac{z(g_{k,k})^2(N_c - 1)}{\pi^2 c N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right)\right],
\label{eq:plusd}
\end{equation}
which reaches a fixed point at very large values of the argument thanks to the $\tanh$
\begin{equation}
\overline{\lambda}^{\mathrm{I}; (+),(d)}_{k}\left( \sqrt{\frac{z(g_{k,k})^2(N_c - 1)}{\pi^2 c N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right)\to\pm\infty\right) = -\frac{2\Lambda_f (g_{k,k})^2(N_c^2-1)}{c N_c N_f} \pm 4\pi\Lambda_f\sqrt{\frac{z(g_{k,k})^2(N_c - 1)}{c N_c N_f}},
\end{equation}
when
\begin{equation}
\pm \ell \gg \sqrt{\frac{\pi^2 c N_c N_f}{z(g_{k,k})^2(N_c - 1)}} \pm 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0,
\end{equation}
where + corresponds to the case $\ell$ positive and - corresponds to $\ell$ negative. The boundary equation for $\mathcal{C}_0$ is
\begin{equation}
\mathcal{C}_0 = -\frac{1}{4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c - 1)(g_{k,k})^2}}\tanh^{-1}\left[\frac{1}{4\pi\Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c - 1)(g_{k,k})^2}}\left( \overline{\lambda}^{\mathrm{I}; (+),(d)}_{k}(0) + \frac{2\Lambda_f (g_{k,k})^2 (N_c^2 - 1)}{c N_c N_f}\right)\right].
\label{eq:plusdinitial}
\end{equation}
Since $\abs{\tanh(x)} < 1$ for real $x$ ,this equation is valid for any real values of $\overline{\lambda}^{\mathrm{I}; (+),(d)}_{k}(0)$. If we allow the range of of $\tanh$ in Eq. \eqref{eq:plusd} to go above 1, i.e. $\abs{\tanh(x)} > 1$, with $\tanh(x)$ real, then the $\tanh^{-1}$ in Eq. \eqref{eq:plusdinitial} will have a $\pi/2$ imaginary part. This $i \pi/2$ term will transform the $\tanh$ in Eq. \eqref{eq:plusd} into a $\coth$, but will keep $\overline{\lambda}^{\mathrm{I}; (+),(d)}_{k}(\ell)$ real.

This is also the case for the $s$-wave, singlet channel:
\begin{equation}
\overline{\lambda}^{\mathrm{I}; (-),(s)}_{k}(\ell) = -\frac{2\Lambda_f (g_{k,k})^2(N_c^2 - 1)}{c N_c N_f} + 4\pi\Lambda_f\sqrt{\frac{z(g_{k,k})^2(N_c + 1)}{c N_c N_f}}\tanh\left[\sqrt{\frac{z(g_{k,k})^2(N_c + 1)}{\pi^2 N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right)\right],
\label{eq:minuss}
\end{equation}
which reaches a fixed point at very large values of the argument
\begin{equation}
\overline{\lambda}^{\mathrm{I}; (-),(s)}_{k}\left( \sqrt{\frac{z(g_{k,k})^2(N_c + 1)}{\pi^2 N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right) \to \pm \infty \right) = -\frac{2\Lambda_f (g_{k,k})^2}{c N_c N_f} \pm 4\pi\Lambda_f\sqrt{\frac{z(g_{k,k})^2(N_c + 1)}{c N_c N_f}},
\end{equation}
when
\begin{equation}
\pm \ell \gg \sqrt{\frac{c N_c N_f}{z(g_{k,k})^2(N_c + 1)}} \pm 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0,
\end{equation}
where again + corresponds to the case $\ell$ positive and - corresponds to $\ell$ negative. The boundary equation for $\mathcal{C}_0$ is
\begin{equation}
\mathcal{C}_0 = -\frac{1}{4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c + 1)(g_{k,k})^2}}\tanh^{-1}\left[\frac{1}{4\pi\Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c + 1)(g_{k,k})^2}}\left( \overline{\lambda}^{\mathrm{I}; (+),(d)}_{k}(0) + \frac{2\Lambda_f (g_{k,k})^2 (N_c^2 - 1)}{c N_c N_f}\right)\right].
\label{eq:minussinitial}
\end{equation}

For the $s$-wave, triplet channel we have
\begin{equation}
\overline{\lambda}^{\mathrm{I}; (+),(s)}_{k}(\ell) = -\frac{2\Lambda_f (g_{k,k})^2(N_c^2 - 1)}{c N_c N_f} - 4\pi\Lambda_f\sqrt{\frac{z(g_{k,k})^2(N_c - 1)}{c N_c N_f}}\tan\left[\sqrt{\frac{z(g_{k,k})^2(N_c - 1)}{\pi^2 c N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right)\right],
\label{eq:pluss}
\end{equation}
with boundary conditions determined by
\begin{equation}
\mathcal{C}_0 = \frac{1}{4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c - 1)(g_{k,k})^2}}\tan^{-1}\left[\frac{1}{4\pi\Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c - 1)(g_{k,k})^2}}\left( \overline{\lambda}^{\mathrm{I}; (+),(s)}_{k}(0) + \frac{2\Lambda_f (g_{k,k})^2 (N_c^2 - 1)}{c N_c N_f}\right)\right].
\label{eq:plussinitial}
\end{equation}
Here, $\overline{\lambda}^{\mathrm{I}; (+),(s)}_{k}(0)$ can take any real values. In this case, the four-fermion coupling diverges at half-integer multiples of $\pi$ in the argument of $\tan$. therefore, the critical values are
\begin{equation}
\ell^{(1);(+),(s)}_c (n) = \pi^2\sqrt{\frac{c N_c N_f}{z(g_{k,k})^2(N_c - 1)}}\left(n - \frac{1}{2}\right) + 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0, \qquad n \in \mathbb{Z}.
\end{equation}
More precisely, we take $\ell^{(1);(+),(s)}_c (1)$ as the critical value. Analogously, for the $d$-wave, singlet channel we have.
\begin{equation}
\overline{\lambda}^{\mathrm{I}; (-),(d)}_{k}(\ell) = -\frac{2\Lambda_f (g_{k,k})^2(N_c^2 - 1)}{c N_c N_f} - 4\pi\Lambda_f\sqrt{\frac{z(g_{k,k})^2(N_c + 1)}{c N_c N_f}}\tan\left[\sqrt{\frac{z(g_{k,k})^2(N_c + 1)}{\pi^2 c N_c N_f}}\left(\ell - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right)\right],
\label{eq:minusd}
\end{equation}
with boundary conditions determined by
\begin{equation}
\mathcal{C}_0 = \frac{1}{4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c + 1)(g_{k,k})^2}}\tan^{-1}\left[\frac{1}{4\pi\Lambda_f}\sqrt{\frac{c N_c N_f}{z(N_c + 1)(g_{k,k})^2}}\left( \overline{\lambda}^{\mathrm{I}; (-),(d)}_{k}(0) + \frac{2\Lambda_f (g_{k,k})^2 (N_c^2 - 1)}{c N_c N_f}\right)\right],
\label{eq:minusdinitial}
\end{equation}
and
\begin{equation}
\ell^{(1);(-),(d)}_c (n) = \pi^2\sqrt{\frac{c N_c N_f}{z(g_{k,k})^2(N_c + 1)}}\left(n - \frac{1}{2}\right) + 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0, \qquad n \in \mathbb{Z}.
\end{equation}
We again have $\ell^{(1);(-),(d)}_c (1)$ as the critical value.

Near the hot spot, i.e. $g_{k,k} = g_{0,0}$, the critical temperature is, for the singlet $d$-wave:
\begin{equation}
T_c^{(-),d} \sim \Lambda_f \exp\left\lbrace -\frac{\pi^2}{2}\sqrt{\frac{2 N_c N_f}{\pi z(N_c + 1)w}} - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right\rbrace,
\end{equation}
where we have used $\ell = \log(\Lambda_f/\mu)$ and $w = v_0/c = 2(g_{0,0})^2/(\pi c)$. For the triplet, $s$-wave:
\begin{equation}
T_c^{(+),s} \sim \Lambda_f \exp\left\lbrace -\frac{\pi^2}{2}\sqrt{\frac{2 N_c N_f}{\pi z(N_c - 1)w}} - 4 c^2 N_c^2 N_f^2 \pi^2 \Lambda_f \mathcal{C}_0 \right\rbrace.
\end{equation}
The fixed points of the other two channels are reached in $\ell \to \infty$, then $T_c^{(+),d} \sim 0$ and $T_c^{(-),s} \sim 0$.












\subsubsection{Absence of perturbative fixed point}
%{$\lambda^{(3)}$ solution}
%
We start with Eq. (119) of the paper,
%
\begin{align}
\frac{\partial}{\partial\ell}\hat\lambda^{(3)\lbrace N_i \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace} = -\hat\lambda^{(3)\lbrace N_i \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace} - x_i\frac{\partial}{\partial x_i} \hat\lambda^{(3)\lbrace N_i \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace} + {S}^{\lbrace N_i \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace}~,
\end{align}
%
The solution for the above equation is given to be,
%
\begin{align}
\hat\lambda^{(3)\lbrace N_i \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace}= \frac{1}{x}\int_{xe^{-\ell}}^x
\mathrm{d}x^{\prime} {S}^{\lbrace N_i \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x^{\prime}\hat x_i \rbrace}
\left(\ell - \log\left[\frac{x}{x^{\prime}}\right]\right)~.
\end{align}
%
At sufficiently large length scale, the momentum dependent coupling becomes important. 
The off-diagonal Yukawa coupling is given as,
\begin{align}
 g_{k^{\prime},k}\left(\ell\right) = 
		\begin{cases}
\sqrt{\FR{\pi^3}{4} \frac{N_cN_f}{N_c^2-1}\frac{1}{\left(\ell_0 + \ell\right)\log\left(\ell_0 + \ell\right)}}		& \ell \le \ell^{(1L)}_{k^{\prime},k} \\
\sqrt{\FR{\pi^3}{4} \frac{N_cN_f}{N_c^2-1}\frac{1}{\left(\ell_0 + \ell^{(1L)}_{k^{\prime},k}\right)\log\left(\ell_0 + \ell^{(1L)}_{k^{\prime},k}\right)}}~ \exp\left(-\FR{\sqrt{\ell+\ell_0}-\sqrt{\ell^{(1L)}_{k^{\prime},k}+\ell_0}}{\sqrt{N_c^2-1}}\right)		& \ell^{(1L)}_{k^{\prime},k} \le \ell 
	\end{cases}~,
		\label{eq:gofffinal1}
\end{align}
%
where, $\ell^{(1L)}_{k^{\prime},k} = {\rm min}\left({\ell^{(2L)}_{(k^{\prime}+k)/2}}, {\ell^{(1L)}_{k^{\prime}}},{\ell^{(1L)}_{k}}\right)\implies$
%
\begin{align}
\ell^{(1L)}_{k^{\prime},k} = {\rm min}\lbrace\log\left(\frac{2\Lambda_f}{v(0;0)|k^{\prime}+k|}\right), ~\log\left(\frac{\Lambda_f}{v(0;0)c(v_0)|k^{\prime}|}\right),~ \log\left(\frac{\Lambda_f}{v(0;0)c(v_0)|k|}\right)\rbrace~.
\end{align}
%
For our purpose, we only need the following forms for the Yukawa coupling,
%
\begin{eqnarray}
g_{0,0}\left(\ell\right) &=& \sqrt{\FR{\pi^3}{4} \frac{N_cN_f}{N_c^2-1}~\frac{1}{\left(\ell_0 + \ell)\right)\log\left(\ell_0 + \ell\right)}}\\
%
g_{0,0}\left(\ell-\log(x/x^{\prime})\right)&\approx& \sqrt{\FR{\pi^3}{4} \frac{N_cN_f}{N_c^2-1}~\frac{1}{\left(\ell_0 + \ell - \log(x/x^{\prime})\right)\log\left(\ell_0 + \ell\right)}}~\\\nonumber
&&~~~~~~~~~\text{(dropping $-\log(x/x^{\prime})$ from the $\log$})\\
%
g_{k^{\prime},k}\left(\ell-\log(x/x^{\prime})\right) &=& g_{0,0}\left(\ell\right)\mathcal{E}_0\left(-\ell_0,\log\left(\frac{2\Lambda_f}{v|k^{\prime}+k|}\right)+\ell\right) \exp\left(-\FR{\sqrt{\ell_0 + \ell - \log(x/x^{\prime})}}{\sqrt{N_c^2-1}}\right)~,
\end{eqnarray}
%
where in the last line, we have used $g_{0,0}(\ell)$, as the $x, x^{\prime}$ dependence is suppressed in the presence 
of the exponential factor.
%
Then, we will encounter mainly three types of integrals involving the form of the Yukawa coupling, given below:
%
\begin{eqnarray}
\int {\mathrm d}x^{\prime} {g_{0,0}\left(\ell-\log(x/x^{\prime})\right)}^4 &&= \left(\FR{\pi^3}{4} \frac{N_cN_f}{N_c^2-1}\right)^2\times\frac{e^{-\ell_0 - \ell} x \text{Ei}\left(\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)\right)-\frac{x^{\prime}}{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}}{\log ^2\left(\ell_0 + \ell\right)},\\
&&= {g_{0,0}}^4\cdot\left(\ell+\ell_0\right)^2\left[e^{-\ell_0 - \ell} x \text{Ei}\left(\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)\right)-\frac{x^{\prime}}{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}\right]~.%
\\\nonumber
%
\int {\mathrm d}x^{\prime} e^{-a\sqrt{\ell_0 + \ell - \log(x/x^{\prime})}} &&= x^{\prime} e^{-a \sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}}-\frac{1}{2} \sqrt{\pi } a x e^{-\frac{a^2}{4} -\ell_0 - \ell} \text{erfi}\left(\frac{a}{2}-\sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}\right),a>0\\
%
&&\approx x^{\prime} e^{-a \sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}}~.\\
%
%
\int {\mathrm d}x^{\prime}~ \frac{e^{-a\sqrt{\ell_0 + \ell - \log(x/x^{\prime})}}}{x^{\prime}} &&= -\frac{2 e^{-a \sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}} \left(a \sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}+1\right)}{a^2},\\
%
&&\approx-\frac{2 e^{-a \sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}}  \sqrt{\ell_0 + \ell-\log \left(\frac{x}{x^{\prime}}\right)}}{a}~.\\\nonumber
%
%
\int {\mathrm d}x^{\prime}~ \frac{e^{-a\sqrt{\ell_0 + \ell - \log(x/x^{\prime})}}}{x^{\prime}}\log(p x^{\prime}) &&= -\frac{2 e^{-a \sqrt{\ell_0 + \ell-\log (x/x^{\prime})}}}{a^4}\Bigg[a \left(\sqrt{\ell_0 + \ell - \log(x/x^{\prime})} \left(a^2 \log (p x^{\prime})+6\right)+a \log (p x^{\prime})\right)\\
&&+2 a^2 \left(\ell_0 + \ell - \log(x/x^{\prime})\right)+6\Bigg]~,\\\nonumber
%
&&\approx -\frac{2 e^{-a \sqrt{\ell_0 + \ell-\log (x/x^{\prime})}} \left(a \log (p x^{\prime})\sqrt{\ell_0 + \ell-\log (x/x^{\prime})} + 2\ell_0 + 2\ell-2\log (x/x^{\prime})\right)}{a^2}~.\\
%
%
\end{eqnarray}
%
%$-\frac{2 e^{-a \sqrt{l+l_0-\log (x)+\log (y)}} \left(a \left(\left(a^2 \log (p y)+6\right) \sqrt{l+l_0-\log (x)+\log (y)}+a \log (p)+3 a \log (y)\right)+2 a^2 \left(l+l_0-\log (x)\right)+6\right)}{a^4}$
%
\subsubsection{$\hat\lambda^{(3)\lbrace 11 \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace}$}
%
\subsubsection{Away from the plane, along $Q_x >0$} %and $v(k_x+p_x) >\Lambda_f, v(k_x-p_x) > \Lambda_f$}
Source term for 11,18 channel can be written as,
%
Integrating, we get,
%
\begin{align}
\hat\lambda^{(3)\lbrace 11,18 \rbrace;\lbrace \sigma_i \rbrace}_{\lbrace x_i \rbrace}=
\begin{cases}
~\dfrac{{g_{0,0}}^4}{16c(v_0)}\left(1-e^{-\ell}\right)~~,&x \leq \Lambda_f/v\\
\\
~\dfrac{{g_{0,0}}^4}{16c(v_0)}\left(\dfrac{\Lambda_f}{vx}-e^{-\ell}\right) ~,&\Lambda_f/c(v_0) < x \leq \Lambda_f/v\\
\end{cases}
\end{align}
%
%
%Source term for 14,15 channel can be written as,
%
\begin{align}
S_{14,15} = 
%
\begin{cases}
~-\dfrac{{g_{0,0}}^4}{16c(v_0)}~,&0< x \leq \Lambda_f/c(v_0)\\
\\
~ -\dfrac{{g_{0,0}}^4}{\pi^2c(v_0)}\dfrac{\Lambda_f}{c(v_0)x}\log\left(\dfrac{2c(v_0)x}{\Lambda_f}\right)~,&\Lambda_f/c(v_0) < x \leq \Lambda_f/v\\
\\
~-\dfrac{{g_{x,0}}^2{g_{0,0}}^2}{\pi^2c(v_0)}\dfrac{\Lambda_f}{c(v_0)x}\log\left(\dfrac{2c(v_0)x}{\Lambda_f}\right)~,&\Lambda_f/v < x\\
\end{cases}
\end{align}
%

\begin{align}
S_{14,15} = 
-\frac{{g_{0,0}}^4}{16c(v_0)}\Theta\left(\frac{\Lambda_f}{c(v_0)}-x|\hat x|\right) - \frac{{g_{0,0}}^4}{\pi^2c(v_0)}~
\frac{\Lambda_f}{c(v_0)x}\log\left(\frac{2c(v_0)x|\hat l|}{\Lambda_f}\right)\Theta\left(\frac{\Lambda_f}{v}-x|\hat x|\right)\Theta\left(x|\hat x|-\frac{\Lambda_f}{c(v_0)}\right)~,
\end{align}








%Counter terms are chosen so that the IR singularity is removed in the vertex function,
%%
%%Once we implement these renormalization conditions for the quantum correction we are able to compute the counter terms $A^{\lambda}_{(n)}$, where $n=0,1,2$ is the order of the four fermion coupling of the quantum correction. These are related by
%\begin{equation}
%A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(n)}(\{ k_i \}) = -\frac{4\mu}{\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_i\}}}\left.\mathbf{\Gamma}^{\{N_i\};\{\sigma_i\}}_{(n)}(\{ {\bf k}_i \})\right|_{\mathbf{k}_i^*} + (\text{regular terms}),
%\end{equation}
%where $A^{\lambda}_{(n)}$ denotes the counter term coefficient that is $n$-th power of $\lambda$.
%The contribution to the beta function is given by the derivative of $A^{\lambda}_{(n)}$,
%\begin{equation}
%\frac{\partial A^{\lambda, \{ N_i \}; \{ \sigma_i \} }_{(n)}(\{ k_{i} \})}{\partial\log\mu}\lambda^{ \{ N_i \} ;\{ \sigma_i \}}_{\{k_{i}\}} = - 4\mu\frac{\partial \mathbf{\Gamma}^{ \{ N_i \}; \{ \sigma_i \} }_{(n)}(\{ {\bf k}_{i} \})}{\partial\log\mu}.
%\end{equation}



\subsection{Construction of the Beta Functions for the $\lambda$ Coupling.}

The beta function is obtained from the equation for the bare coupling
\begin{equation}
\lambda^{\mathsf{B},\{ N_i \}; \{\sigma_i \}}_{\{k^{\mathsf{B}}_{i, N_i} \}} = \mu^{-1}Z_{\tau}^{-3}\left[ \prod_{j=1}^4 Z^{(\psi )}(k_{j, N_j}) \right]^{-1/2} Z^{\lambda, \{ N_i \}; \{\sigma_i \}}(\{k_{i, N_i} \})\lambda^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}},
\label{eq:bare}
\end{equation}
where the bare quantities are independent of $\mu$. The counter-term $Z^{\lambda, \{ N_i \}; \{\sigma_i \}}(\{k_{i, N_i} \}) = 1 + A^{\lambda, \{ N_i \}; \{\sigma_i \}}(\{k_{i, N_i} \})$, and we can expand $A^{\lambda, \{ N_i \}; \{\sigma_i \}}(\{k_{i, N_i} \})$ in powers of $\lambda$:
\begin{equation}
A^{\lambda, \{ N_i \}; \{\sigma_i \}}(\{k_{i, N_i} \}) = A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \}) + A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \}) + A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(2)}(\{k_{i, N_i} \}),
\end{equation}
where $A_{(0)}$, $A_{(1)}$ and $A_{(2)}$ are the counter terms independent, linear and quadratic in $\lambda$, respectively. 
We need to express Eq. \eqref{eq:bare} in terms of the dimensionful four fermion coupling $\overline{\lambda} = \mu^{-1}\lambda$, which is irrelevant and independent of $\mu$, and define the quantities
\begin{align}
Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \}) = & Z_{\tau}^{-3}\left[ \prod_{j=1}^4 Z^{(\psi )}(k_{j, N_j}) \right]^{-1/2} A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})\overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}}, \label{eq:z0lambda}
\\ Z^{g_i, \lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \}) = & Z_{\tau}^{-3}\left[ \prod_{j=1}^4 Z^{(\psi )}(k_{j, N_j})\right]^{-1/2}\left[ 1 + A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \}) + A^{\lambda, \{ N_i \}; \{\sigma_i \}}_{(2)}(\{k_{i, N_i} \}) \right].\label{eq:z1lambda}
\end{align}
Therefore, we can write Eq. \eqref{eq:bare} as 
\begin{equation}
\lambda^{\mathsf{B},\{ N_i \}; \{\sigma_i \}}_{\{k^{\mathsf{B}}_{i, N_i} \}} = Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})\overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}} + Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \}),
\label{eq:barez0z1}
\end{equation}
where $Z_{(0)}$ is $\lambda$-independent and $Z_{(1)}$ is $\lambda$-dependent and $g_i$ represents the $v, V_F$ and $g$ couplings.

We can take the $\mu$-derivative of this quantity and obtain:
\begin{equation}
\begin{aligned}
0 = & Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})\beta^{(\overline{\lambda});\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}} + \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}}\left[ \int \dd x_j \dd x_k \frac{\delta Z^{g_i,\lambda , \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\delta g_i(x_j,x_k)}\beta^{(g_i)}_{x_j,x_k} \right.
\\ & \left. + \int \left( \prod_{j=1}^4 \dd x_j \right)\frac{\delta Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\delta \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{ x_j \}} }\beta^{(\overline{\lambda});\{ N_i \}; \{\sigma_i \}}_{\{ x_j \}} + \frac{\partial Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\partial\log\mu} \right]
\\ & + \int \dd x_j \dd x_k \frac{\delta Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})}{\delta g_i(x_j, x_k)}\beta^{(g_i)}_{x_j, x_k} + \frac{\partial Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})}{\partial\log\mu}.
\end{aligned}
\end{equation}
Next, we can solve for $\beta^{(\overline{\lambda});\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}} = \int \left( \prod_{j=1}^4 \dd x_j \delta(x_j - k_{i, N_i}) \right) \beta^{(\overline{\lambda});\{ N_i \}; \{\sigma_i \}}_{\{ x_j \}}$
\begin{equation}
\begin{aligned}
& \left [Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \}) \int \left( \prod_{j=1}^{4}\dd x_j \delta(x_j - k_{i, N_i}) \right) + \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}}\int \left( \prod_{j=1}^4 \dd x_j \right)\frac{\delta Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\delta \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{ x_j \}} } \right]\beta^{(\overline{\lambda});\{ N_i \}; \{\sigma_i \}}_{\{ x_j \}}
\\ = & - \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}}\left[ \int \dd x_j \dd x_k \frac{\delta Z^{g_i,\lambda , \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\delta g_i(x_j,x_k)}\beta^{(g_i)}_{x_j,x_k} + \frac{\partial Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\partial\log\mu} \right]
\\ & - \int \dd x_j \dd x_k \frac{\delta Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})}{\delta g_i(x_j, x_k)}\beta^{(g_i)}_{x_j, x_k} - \frac{\partial Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})}{\partial\log\mu}.
\end{aligned}
\label{eq:betafull}
\end{equation}
To simplify the expression we can add and subtract 1 to $Z^{g_i,\lambda}_{(1)}$ in the left hand side and notice that the functional derivatives are equivalent in order to the partial derivatives with respect to the functions, i.e. $\int \delta/\delta\mathsf{A} \equiv \partial/\partial\mathsf{A}$, with $\mathsf{A}$ any coupling. Using this we can state the following inequalities
\begin{subequations}
\begin{align}
\int \dd x_j \dd x_k g_i(x_j,x_k) \frac{\delta Z^{g_i,\lambda}_{(1)}}{\delta g_i(x_j,x_k)}\frac{\beta^{(g_i)}_{x_j,x_k}}{g_i(x_j,x_k)} \sim \mathcal{O}\left( w \int \dd x_j \dd x_k g_i(x_j,x_k) \frac{\delta Z^{g_i,\lambda}_{(1)}}{\delta g_i(x_j,x_k)} \right) \sim\mathcal{O}\left( w Z^{g_i,\lambda}_{(1)} \right) & \ll \frac{\partial Z^{g_i,\lambda}_{(1)}}{\partial\log\mu}, \label{eq:zordera}
\\ \int \dd x_j \dd x_k g_i(x_j,x_k) \frac{\delta Z^{g_i,\lambda}_{(0)}}{\delta g_i(x_j,x_k)}\frac{\beta^{(g_i)}_{x_j,x_k}}{g_i(x_j,x_k)} \sim \mathcal{O}\left( w \int \dd x_j \dd x_k g_i(x_j,x_k) \frac{\delta Z^{g_i,\lambda}_{(0)}}{\delta g_i(x_j,x_k)} \right) \sim\mathcal{O}\left( w Z^{g_i,\lambda}_{(0)} \right) & \ll \frac{\partial Z^{g_i,\lambda}_{(0)}}{\partial\log\mu}, \label{eq:zorderb}
\\ \left( Z^{g_i,\lambda}_{(1)} - 1 \right), \ \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{ k_{i,N_i} \}}\left( \int\prod_{j=1}^4 \dd x_j \right)\frac{\delta Z^{g_i,\lambda}_{(1)}}{\delta \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{ x_j \}}} \sim \mathcal{O}\left( w \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{ k_{i,N_i} \}} \right) & \ll 1. \label{eq:zorderc}
\end{align}
\label{eq:zorder}
\end{subequations}
Applying these inequalities to Eq. \eqref{eq:betafull}
\begin{equation}
\beta^{(\overline{\lambda});\{ N_i \}; \{\sigma_i \}}_{\{ k_{i,N_i} \}} = - \overline{\lambda}^{\{ N_i \}; \{\sigma_i \}}_{\{k_{i, N_i} \}} \frac{\partial Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\partial\log\mu} - \frac{\partial Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})}{\partial\log\mu}.
\label{eq:betasimple}
\end{equation}
This quantity is very simple, but it is still not the one we want. What we are looking for is the beta function of $\lambda$, which in terms of the beta function we just found is, is $\beta^{(\overline{\lambda})} = \mu^{-1}\beta^{(\lambda)} - \mu^{-1}\lambda$, with $\beta^{(\lambda)} = \frac{\dd \lambda}{\dd\log\mu}$. Simplifying Eq. \eqref{eq:betasimple} with this expression gives us
\begin{equation}
\beta^{(\lambda);\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}} = \frac{\dd\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}}}{\dd\log\mu} = \left( 1 - \frac{\partial Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\partial\log\mu}\right)\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}} - \mu \frac{\partial Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \})}{\partial\log\mu}.
\label{eq:prebetalambda}
\end{equation}

In order to proceed we need to take a deeper look at Eqs. \eqref{eq:z0lambda} and \eqref{eq:z1lambda}. Let us begin with the latter one. For the $\log\mu$ derivative of this expression, when multiplied by $\overline{\lambda}$ as in Eq. \eqref{eq:prebetalambda}, we wish to keep terms of order $w \lambda$ and order $\lambda^2$ and neglect the rest. We already know that $A^{\lambda}_{(1)} \sim \mathcal{O}[w(k_{i,N_i})]$ and $\lambda A^{\lambda}_{(2)} \sim \mathcal{O}[\lambda(k_{i,N_i})^2]$. To see what other terms to keep, let us write $\partial Z_{(1)}/\partial\log\mu$ more explicitly,
\begin{equation}
\begin{aligned}
\frac{\partial Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\partial\log\mu} = & -3 Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \}) \frac{\partial \log Z_\tau}{\partial\log\mu} - \frac{1}{2} Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})\sum_{j=1}^4 \frac{\partial \log Z^{(\psi)}(k_{j,N_j})}{\partial\log\mu} 
\\ & + Z_{\tau}^{-3} \left[\prod_{j=1}^4 Z^{(\psi)}(k_{j,N_j})\right]^{-1/2} \left[ \frac{\partial A^{\lambda, \{N_i\};\{\sigma_i\}}_{(1)}(\{k_{i,N_i}\})}{\partial\log\mu} + \frac{\partial A^{\lambda, \{N_i\};\{\sigma_i\}}_{(2)}(\{k_{i,N_i}\})}{\partial\log\mu} \right].
\end{aligned}
\label{eq:prez1term}
\end{equation}
Writing the momentum-dependent scaling factors as they are defined below Eq. \eqref{eq:RenormalizedQuantities} we can conclude on the order of $\partial \log Z_\tau/\partial\log\mu$ and $\partial \log Z^{(\psi)}/\partial\log\mu$:
\begin{equation}
Z_\tau = \frac{1+A^{(1)}(0)}{1 + A^{(3)}(0)} = 1 + \mathcal{O}[w(0))], \qquad Z^{(\psi)}(k_{i,N_i}) = \frac{1 + A^{(1)}(k_{i,N_i})}{Z_\tau^2} = 1 + \mathcal{O}[w(k_{i,N_i})],
\end{equation}
which implies
\begin{equation}
\frac{\partial \log Z_\tau}{\partial \log\mu} = \frac{1}{Z_\tau}\frac{\partial Z_\tau}{\partial \log\mu} = \mathcal{O}[w(0)], \qquad \frac{\partial \log Z^{(\psi)}(k_{i,N_i})}{\partial\log\mu} = \frac{1}{Z^{(\psi)}(k_{i,N_i})}\frac{\partial Z^{(\psi)}(k_{i,N_i})}{\partial\log\mu}= \mathcal{O}[w(k_{i,N_i})],
\label{eq:scalingorders}
\end{equation}
and
\begin{equation}
Z_{\tau}^{-3} \left[\prod_{j=1}^4 Z^{(\psi)}(k_{j,N_j})\right]^{-1/2} = 1+ \mathcal{O}[w(0), w(k_{i,N_i})].
\label{eq:scalingmultorders}
\end{equation}
These statements help us to retroactively prove Eqs. \eqref{eq:zorder} and together with Eq. \eqref{eq:zorderc} to simplify Eq. \eqref{eq:prez1term} with the result
\begin{equation}
\begin{aligned}
\frac{\partial Z^{g_i,\lambda, \{ N_i \}; \{\sigma_i \}}_{(1)}(\{k_{i, N_i} \})}{\partial\log\mu} = & -3 \frac{\partial \log Z_\tau}{\partial\log\mu} - \frac{1}{2}\sum_{j=1}^4 \frac{\partial \log Z^{(\psi)}(k_{j,N_j})}{\partial\log\mu} 
\\ & + \frac{\partial A^{\lambda, \{N_i\};\{\sigma_i\}}_{(1)}(\{k_{i,N_i}\})}{\partial\log\mu} + \frac{\partial A^{\lambda, \{N_i\};\{\sigma_i\}}_{(2)}(\{k_{i,N_i}\})}{\partial\log\mu}.
\end{aligned}
\label{eq:z1term}
\end{equation}
where:
\begin{align}
\frac{\partial A^{\lambda, \{ N_i \}; \{ \sigma_i \} }_{(1)}(\{ k_{i,N_i} \})}{\partial\log\mu}\lambda^{ \{ N_i \} ;\{ \sigma_i \}}_{\{k_{i,N_i}\}} = & - 4\mu\frac{\partial \mathbf{\Gamma}^{ \{ N_i \}; \{ \sigma_i \} }_{(1)}(\{ k_{i,N_i} \})}{\partial\log\mu}, \label{eq:z1termA}
\\ \frac{\partial A^{\lambda, \{ N_i \}; \{ \sigma_i \} }_{(2)}(\{ k_{i,N_i} \})}{\partial\log\mu}\lambda^{ \{ N_i \} ;\{ \sigma_i \}}_{\{k_{i,N_i}\}} = & - 4\mu\frac{\partial \mathbf{\Gamma}^{ \{ N_i \}; \{ \sigma_i \} }_{(2)}(\{ k_{i,N_i} \})}{\partial\log\mu}, \label{eq:z2termA}
\end{align}
as expected since $\overline{\lambda}$ is independent of $\mu$.

Now we move to the term $\mu \partial Z_{(0)}/\partial\log\mu$ in Eq. \eqref{eq:prebetalambda}. The full term is
\begin{equation}
\begin{aligned}
\mu \frac{\partial Z^{g_i, \{ N_i \}; \{\sigma_i \} }_{(0)}(\{k_{i, N_i} \})}{\partial\log\mu} = & - 3 \mu Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{k_{i, N_i} \}) \frac{\partial \log Z_\tau}{\partial\log\mu} - \frac{\mu}{2} Z^{g_i, \{ N_i \}; \{\sigma_i \}}_{(0)}(\{ k_{i, N_i} \})\sum_{j=1}^4 \frac{\partial \log Z^{(\psi)}(k_{j,N_j})}{\partial\log\mu} 
\\ & + Z_{ \tau }^{-3} \left[\prod_{j=1}^4 Z^{(\psi)}(k_{j,N_j})\right]^{-1/2} \frac{\partial A^{\lambda, \{ N_i \}; \{ \sigma_i \} }_{(0)}(\{ k_{i,N_i} \})}{\partial\log\mu}\lambda^{ \{ N_i \} ;\{ \sigma_i \}}_{\{k_{i,N_i}\}}.
\end{aligned}
\label{eq:prez0term}
\end{equation}

We know that $A^{\lambda}_{(0)} \lambda \sim \mathcal{O}[w(k_{i,N_i})^3]$, and for this source term we want to keep the terms of this order. Using Eqs. \eqref{eq:zorderb}, \eqref{eq:scalingorders} and \eqref{eq:scalingmultorders} we can neglect all the terms of the first line since they are of order $w^4$. Likewise, we use Eq. \eqref{eq:scalingmultorders} keep the term of order $w^3$ in the second line. The result is 
\begin{equation}
\mu \frac{\partial Z^{g_i, \{ N_i \}; \{\sigma_i \} }_{(0)}(\{k_{i, N_i} \})}{\partial\log\mu} = \frac{\partial A^{\lambda, \{ N_i \}; \{ \sigma_i \} }_{(0)}(\{ k_{i,N_i} \})}{\partial\log\mu}\lambda^{ \{ N_i \} ;\{ \sigma_i \}}_{\{k_{i,N_i}\}} = - 4\mu\frac{\partial \mathbf{\Gamma}^{ \{ N_i \}; \{ \sigma_i \} }_{(0)}(\{ k_{i,N_i} \})}{\partial\log\mu}.
\label{eq:z0term}
\end{equation}

Simplifying Eq. \eqref{eq:prebetalambda} with Eqs. \eqref{eq:z1term} and \eqref{eq:z0term} we obtain the beta function for the four-fermion coupling:
\begin{equation}
\begin{aligned}
\beta^{(\lambda);\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}} = & \left( 1 + 3 \frac{\partial \log Z_\tau}{\partial\log\mu} + \frac{1}{2}\sum_{j=1}^4 \frac{\partial \log Z^{(\psi)}(k_{j,N_j})}{\partial\log\mu} \right)\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}}
\\ & -\frac{\partial A^{\lambda, \{N_i\};\{\sigma_i\}}_{(1)}(\{k_{i,N_i}\})}{\partial\log\mu}\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}} - \frac{\partial A^{\lambda, \{N_i\};\{\sigma_i\}}_{(2)}(\{k_{i,N_i}\})}{\partial\log\mu}\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}}
\\ & - \frac{\partial A^{\lambda, \{ N_i \}; \{ \sigma_i \} }_{(0)}(\{ k_{i,N_i} \})}{\partial\log\mu}\lambda^{ \{ N_i \} ;\{ \sigma_i \}}_{\{k_{i,N_i}\}},
\end{aligned}
\label{eq:betalambda}
\end{equation}
where $\partial_{\log\mu} \log Z_\tau$ and $\partial_{\log\mu} \log Z^{(\psi)}$ are the leading orders of the dynamical critical exponent $z-1$ and the anomalous scaling dimension of the fermionic field $\eta^{(\psi)}$, respectively. This equation can be written in a simplified way using Eqs. \eqref{eq:z1termA}, \eqref{eq:z2termA} and \eqref{eq:z0term} as
\begin{equation}
\beta^{(\lambda);\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}} = \left( 1 + 3 \frac{\partial \log Z_\tau}{\partial\log\mu} + \frac{1}{2}\sum_{j=1}^4 \frac{\partial \log Z^{(\psi)}(k_{j,N_j})}{\partial\log\mu} \right)\lambda^{\{N_i\};\{\sigma_i\}}_{\{k_{i,N_i}\}} + 4\mu \sum_{j = 0}^{2}\frac{\partial \mathbf{\Gamma}^{ \{ N_i \}; \{ \sigma_i \} }_{(j)}(\{ k_{i,N_i} \})}{\partial\log\mu}
\label{eq:betalambda2}
\end{equation}

Comparing Eqs. \eqref{eq:betalambda} or \eqref{eq:betalambda2} with Eq. \eqref{eq:beta_4f}, the first term of the first line is a contribution that arises from our choice of interaction-driven scaling and does not affects the physics of the problem. The other terms of the first line, together with the first term in the second line contain the $\lambda$-linear terms coming from the vertex corrections in Fig. \ref{fig:4f1}. The last term in the second line contains the BCS corrections in Fig \ref{fig:4f2}. Finally, the last term in the last line is the source term, coming from the four-fermion coupling that is generated in Fig. \ref{fig:4f0}. In Eq. \eqref{eq:beta_4f}, the derivative is take with respect to $\ell = \log\left( \Lambda_f /\mu \right)$, hence the sign differences.

















\section{Old version : Beta functionals for shifted four-fermion couplings }
\label{sec:shiftedffc_old}




With
\begin{equation}
\tilde{\lambda}^{\mathrm{I};\spmqty{\alpha & \beta \\ \delta & \gamma}}_{\spmqty{K_1 & -K_1 \\ K_2 & -K_2}} = \frac{1}{\sqrt{\hat{V}_{F,K_1}\hat{V}_{F,K_2}}}\left(\hat{\lambda}^{\mathrm{I};\spmqty{\alpha & \beta \\ \delta & \gamma}}_{\spmqty{K_1 & -K_1 \\ K_2 & -K_2}} - \frac{2 \mathsf{T}_{\beta \gamma; \alpha \delta}}{N_f}\hat{\mathsf{D}}(K_1; K_2)\right),
\end{equation}
\eq{eq:betabigmatrixsimple_main} can be written as
\begin{equation}
\begin{aligned}
\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P}\right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\frac{1}{2}\left(\frac{\dd\log Z^{(1)}(K)}{\dd\log\mu} + \frac{\dd\log Z^{(3)}(K)}{\dd\log\mu} + \frac{\dd\log Z^{(1)}(P)}{\dd\log\mu} +\frac{\dd\log Z^{(3)}(P)}{\dd\log\mu}\right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & - \frac{1}{4\pi}\int \frac{\dd Q}{2 \pi \Lambda_f}\sum_{\beta, \alpha = 1}^{N_c}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} -\frac{2 \mathsf{T}_{\sigma_2 \sigma_3; \sigma_1 \sigma_4}}{N_f}\mathsf{R}( K, P),
\end{aligned}
\label{eq:betapptilde}
\end{equation}
where 
\begin{equation}
\mathsf{R}( K, P) = \left[ -\frac{\dd}{\dd\log\mu} + \frac{1}{2}\left( \frac{\dd\log Z^{(1)}(K)}{\dd\log\mu} + \frac{\dd\log Z^{(3)}(K)}{\dd\log\mu} + \frac{\dd\log Z^{(1)}(P)}{\dd\log\mu} +\frac{\dd\log Z^{(3)}(P)}{\dd\log\mu} \right) \right]\left(\frac{\hat{\mathsf{D}}(\Lambda_f; K , P)}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\right)
\label{eq:Requation}
\end{equation}
and we use  
%$\hat{\mathsf{D}}(K_1,K_2)=\hat{\mathsf{D}}(K_2,K_1)$ and 
%$\mathsf{T}_{\beta \gamma; \alpha \delta} = \mathsf{T}_{\gamma \beta; \delta \alpha}$ are used. 
%The last term in the previous equation is the quantity of interest, we call it residual term $\mathsf{R}$. Explicitly
%
%Where
\begin{equation}
\left[ \frac{\partial }{\partial\ell} + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right]\left(\frac{\hat{\mathsf{D}}(K , P)}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\right) \equiv -\frac{\dd }{\dd \log\mu}\left(\frac{\hat{\mathsf{D}}(K , P)}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\right) \equiv -\frac{\dd }{\dd \log\Lambda_f}\left(\frac{\hat{\mathsf{D}}(K , P)}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\right).
\end{equation}
To simplify Eq. \eqref{eq:Requation}, we notice that $\hat{\mathsf{D}}$ can be written as $\mathsf{D}\times\spmqty{0 & 1 \\ 1 & 0}$. The elements are $\mathsf{D}(K; P) = \Lambda_f \abs{g_{K,P}}^2 D(\Lambda_f; K, P)$, where $D(\Lambda_f; K, P)^{-1} = \Lambda_f + c\abs{K-P} + c\abs{\hat{v}_K K + \hat{v}_P P} $ is the original boson propagator, like the one defined in Eq. \eqref{eq:bosonscale} (before shifting $q_x$.) The expression for these elements is
\begin{equation}
\begin{aligned}
-\frac{\dd }{\dd \log\mu}\mathsf{D}(K; P) = & -\mu\left[1 + \frac{\dd }{\dd\log\mu} \right] \left[ (\hat{g}_{K, P})^2 D(\Lambda_f; K, P) \right]
\\ = & - \mathsf{D}(K,P) - 2\Lambda_f \hat{g}_{K,P} \beta^{(g)}_{K, P} D(\Lambda_f; K, P) - \Lambda_f (\hat{g}_{K, P})^2 \frac{\dd D(\Lambda_f; K, P)}{\dd\log\mu}.
\end{aligned}
\label{eq:Dderivative}
\end{equation}
Using the beta function of $g$ in Eq. \eqref{eq:newZ3}, we can write the second term of this last expression as
\begin{equation}
\begin{aligned}
& - 2\Lambda_f \hat{g}_{K,P} \beta^{(g)}_{K, P} D(\Lambda_f; K, P)
\\ & \hspace{1.5cm} = \mathsf{D}(K, P)\left(2\frac{\dd \log Z^{(4)}(K, P)}{\dd\log\mu} -2\eta^{(\Phi)} -2\hat{\eta}^{(\psi)}_{K} -2\hat{\eta}^{\psi}(P) - 4(z-1) \right).
\label{eq:Dsecondterm}
\end{aligned}
\end{equation}
For the third term in Eq. \eqref{eq:Dderivative}, we need to see how the $\log\mu$ derivative acts on $D$ more explicitly. To do that, we express the term as
\begin{equation}
-\frac{\dd D(K, P)}{\dd\log\mu} = -\frac{\dd }{\dd\log\mu}\left.\left( D(Q_0 ; K, P)\right)\right|_{Q_0 = \Lambda_f = \mu e^{\ell}}.
\label{eq:Dthirdtermexpression}
\end{equation}
From Eqs. \eqref{eq:RenormalizedQuantities}, we can see that the boson two point function satisfies
\begin{equation}
\left\langle \Phi^{\mathsf{B}}(Q_1^{\mathsf{B}}) \Phi^{\mathsf{B}}(Q_2^{\mathsf{B}}) \right\rangle = Z^{\Phi}\left\langle \Phi(Q_1) \Phi(Q_2) \right\rangle.
\end{equation}
And from
\begin{equation}
\begin{aligned}
\left\langle \Phi^{\mathsf{B}}(Q_1^{\mathsf{B}}) \Phi^{\mathsf{B}}(Q_2^{\mathsf{B}}) \right\rangle \sim & \delta^{(3)}(Q_1^{\mathsf{B}} + Q_2^{\mathsf{B}}) D^{\mathsf{B}}(Q_0^{\mathsf{B}}; Q_1^{\mathsf{B}}, Q_2^{\mathsf{B}}),
\\ \left\langle \Phi(Q_1) \Phi(Q_2) \right\rangle \sim & \delta^{(3)}(Q_1 + Q_2) D(Q_0; Q_1, Q_2),
\end{aligned}
\end{equation}
it is easy to see that $\delta^{(3)}(Q_1^{\mathsf{B}} + Q_2^{\mathsf{B}}) = Z_{\tau}\delta^{(3)}(Q_1 + Q_2)$ (the $Z_{\tau}$ comes from the frequency delta function) and we obtain the following expression
\begin{equation}
D(Q_0; K, P) = \frac{D^{\mathsf{B}}(Q_0^{\mathsf{B}}; K^{\mathsf{B}}, P^{\mathsf{B}})}{Z^{\Phi}Z_{\tau}}.
\end{equation}
We can plug this in Eq. \eqref{eq:Dthirdtermexpression} and use the chain rule obtain
\begin{equation}
\begin{aligned}
& -\frac{\dd }{\dd\log\mu}\left.\left( D(Q_0 ; K, P)\right)\right|_{Q_0 = \Lambda_f}
\\ & = \left( 2\eta^{\Phi} + z-1 \right) D(K, P) - \frac{1}{Z^{\Phi}Z_{\tau}}\left( \frac{\partial Q_0^{\mathsf{B}}}{\partial\log\mu}\frac{\dd }{\dd Q_0^{\mathsf{B}}}D^{\mathsf{B}}(Q_0^{\mathsf{B}}; K^{\mathsf{B}}, P^{\mathsf{B}}) \right)_{Q_0 = \Lambda_f}.
\end{aligned}
\end{equation}
We can use the chain rule again to simplify the last term and obtain
\begin{equation}
-\frac{\dd }{\dd\log\mu}\left.\left( D(Q_0 ; K, P)\right)\right|_{Q_0 = \Lambda_f} = \left( 2\eta^{(\Phi)} + z-1 \right) D(\mu; K, P) - z\frac{\dd D(K, P)}{\dd\log\mu}.
\end{equation}
Putting everything back into Eq. \eqref{eq:Dderivative} gives
\begin{equation}
\begin{aligned}
-\frac{\dd }{\dd \log\mu}\mathsf{D}(K; P)  = & \left( -1-3(z-1)- 2\hat{\eta}^{(\psi)}_{K} - 2\hat{\eta}^{(\psi)}_{P} + 2\frac{\dd\log Z^{(4)}(K, P)}{\dd\log\mu} \right)\mathsf{D}(K; P)
\\ & - \Lambda_f z (\hat{g}_{K, P})^2\frac{\dd D(K , P)}{\dd\log\mu}.
\end{aligned}
\label{eq:Dderivativesimple}
\end{equation}
Substituting this back into Eq. \eqref{eq:Requation}, we obtain
\begin{equation}
\begin{aligned}
\mathsf{R}( K, P) & = \frac{1}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\left(2\frac{\dd\log Z^{(4)}(K, P)}{\dd\log\mu}\hat{\mathsf{D}}(K; P) - \Lambda_f z (\hat{g}_{K, P})^2\frac{\dd \hat{D}(K , P)}{\dd\log\mu}\right)
\\ & \approx - \frac{\Lambda_f z (\hat{g}_{K, P})^2}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\frac{\dd \hat{D}(K , P)}{\dd\log\mu},
\end{aligned}
\label{eq:Requationfinal}
\end{equation}
where $\hat{D}$ is the matrix with boson propagator $D(\Lambda_f; K,P)^{-1} = \Lambda_f + c\left( \abs{K-P} + \abs{\hat{v}_{K} K + \hat{v}_{P} P} \right)$, i.e $\hat{D}(K,P) = D(\Lambda_f; K,P)\spmqty{0 & 1 \\ 1 & 0}$ (as in \eqref{eq:propmatrix}), and the first term containing $Z^{(4)}$ on the second line is sub-leading. We also have used the beta function of $\hat{V}_F$ to simplify the second line of the last equation. The explicit matrix $\mathsf{R}$ is
\begin{equation}
\mathsf{R}( K, P) = \frac{z (\hat{g}_{K, P})^2}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\frac{\Lambda_f^2}{\left(\Lambda_f + c \abs{K -P} + c \abs{\hat{v}_{K}K + \hat{v}_{P}P}\right)^2}\spmqty{0 & 1 \\ 1 & 0}.
\label{eq:newRel}
\end{equation}
The expression for the beta function, with the residual $\mathsf{R}$ is
\begin{equation}
\begin{aligned}
\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P}\right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\frac{1}{2}\left(\frac{\dd\log Z^{(1)}(K)}{\dd\log\mu} + \frac{\dd\log Z^{(3)}(K)}{\dd\log\mu} + \frac{\dd\log Z^{(1)}(P)}{\dd\log\mu} +\frac{\dd\log Z^{(3)}(P)}{\dd\log\mu}\right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & - \frac{1}{4\pi}\int \frac{\dd Q}{2 \pi \Lambda_f}\sum_{\beta, \alpha = 1}^{N_c}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} -\frac{2 \mathsf{T}_{\sigma_2 \sigma_3; \sigma_1 \sigma_4}}{N_f}\mathsf{R}( K, P).
\end{aligned}
\label{eq:betappR}
\end{equation}
Notice that the measure is now
\begin{equation}
\frac{\dd Q}{2\pi\Lambda_f}.
\end{equation}

To proceed, let us define the matrix $\hat{\eta}$ as
\begin{equation}
\hat{\eta}_{\beta \gamma ; \alpha \delta} (K_1,K_2) = \pi \Lambda_f \left( \frac{\dd\log Z^{(1)}(K_1)}{\dd\log\mu} + \frac{\dd\log Z^{(3)}(K_1)}{\dd\log\mu}\right)\delta(K_1 - K_2)\delta_{\beta \gamma}\delta_{\alpha \delta}\spmqty{1 & 0 \\ 0 & 1}.
\label{eq:etamatrix2}
\end{equation}
This way we can express Eq. \eqref{eq:betappR} as
\begin{equation}
\begin{aligned}
\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\sum_{\beta, \alpha = 1}^{N_c}\int \frac{\dd Q}{2\pi\Lambda_f}\left( \tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}} \hat{\eta}_{\beta \sigma_4 ; \alpha \sigma_3}(Q,K)+ \hat{\eta}_{\beta \sigma_1 ; \alpha \sigma_2}(P, Q)\tilde{\lambda}^{\mathrm{I}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}}\right.
\\ & \left. + \frac{1}{4\pi}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} \right)-\frac{2 \mathsf{T}_{\sigma_2 \sigma_3; \sigma_1 \sigma_4}}{N_f}\mathsf{R}( K, P).
\end{aligned}
\label{eq:betaeta}
\end{equation}
We can complete the square as follows
\begin{equation}
\begin{aligned}
\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\sum_{\beta, \alpha = 1}^{N_c}\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{2\sqrt{\pi}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}} + 2\sqrt{\pi}\hat{\eta}_{\beta \sigma_1 ; \alpha \sigma_2}(P, Q) \right)\left( \frac{1}{2\sqrt{\pi}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} + 2\sqrt{\pi}\hat{\eta}_{\beta \sigma_4 ; \alpha \sigma_3}(Q,K) \right)
\\ &  + \sum_{\beta, \alpha = 1}^{N_c}\int \frac{\dd Q}{2\pi\Lambda_f} 4\pi\hat{\eta}_{\beta \sigma_1 ; \alpha \sigma_2}(P, Q)\hat{\eta}_{\beta \sigma_4 ; \alpha \sigma_3}(Q,K) -\frac{2 \mathsf{T}_{\sigma_2 \sigma_3; \sigma_1 \sigma_4}}{N_f}\mathsf{R}( K, P).
\end{aligned}
\label{eq:etabeta}
\end{equation}
We need to find the eigenvalues of the matrix $\hat{\eta}$ and the $\mathsf{R}$ matrix in order to find the eigenvalues of the four-fermion coupling $\tilde{\lambda}$.

We need to express this last equation in more explicit terms, separating the spin symmetric (triplet) and spin anti-symmetric channels and the $d$- and $s$-wave channels in the hot spot indices. The matrix $\hat{\eta}$ is already a diagonal matrix in the momentum indices. Therefore, we only need to write explicitly it in terms of $\Lambda_f$, $c$ and the couplings. To proceed, we first note that
\begin{equation}
\frac{\dd \log Z^{(1)}(K)}{\dd\log\mu} \gg \frac{\dd \log Z^{(3)}(K)}{\dd\log\mu},
\end{equation}
since $1/c \gg \log(1/c)$ in the small c limit (See Eqs. \eqref{eq:allcounterterms}.) In the current limit, the term of the matrix is
\begin{equation}
\frac{\dd \log Z^{(1)}(K)}{\dd\log\mu} = \frac{(\hat{g}_{K,K})^2(N_c^2 -1)}{\pi^2 c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}},
\end{equation}
which means
\begin{equation}
\begin{aligned}
\hat{\eta}_{\sigma_4 \sigma_1; \sigma_3 \sigma_2}(K_1,K_2) = & \pi\Lambda_f \frac{(\hat{g}_{K_1,K_2})^2(N_c^2 -1)}{\pi^2 c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K_1} \abs{K_1}} \delta_{\sigma_4 \sigma_1}\delta_{\sigma_3 \sigma_2}\delta(K_1-K_2)\spmqty{1 & 0 \\ 0 & 1}
\\ = & 2\pi \Lambda_f \frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K_1} \abs{K_1}} w^{(\eta)}_{\sigma_4 \sigma_1; \sigma_3 \sigma_2}(K_1,K_2)\delta(K_1-K_2)\spmqty{1 & 0 \\ 0 & 1},
\end{aligned}
\end{equation}
where
\begin{equation}
w^{(\eta)}_{\sigma_4 \sigma_1; \sigma_3 \sigma_2}(K_1, K_2) = \frac{\left(N_c^2 - 1\right)(\hat{g}_{K_1, K_2})^2}{2\pi^2 c N_c N_f}\delta_{\sigma_4 \sigma_1}\delta_{\sigma_3 \sigma_2}
\end{equation}
is the weight of the $\hat{\eta}$-term (the delta function means $\hat{g}_{K_1,K_2} = \hat{g}_{K_1,K_1}$.) Using this we can eliminate the integral and sum from the second to last term in Eq. \eqref{eq:etabeta}:
\begin{equation}
\begin{aligned}
\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\sum_{\beta, \alpha = 1}^{N_c}\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{2\sqrt{\pi}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}} + 2\sqrt{\pi}\hat{\eta}_{\beta \sigma_1 ; \alpha \sigma_2}(P, Q) \right)\left( \frac{1}{2\sqrt{\pi}}\tilde{\lambda}^{\mathrm{I}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} + 2\sqrt{\pi}\hat{\eta}_{\beta \sigma_4 ; \alpha \sigma_3}(Q,K) \right)
\\ &  + 2 \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta_{\sigma_4 \sigma_1}\delta_{\sigma_3 \sigma_2} \delta(P-K)\spmqty{1 & 0 \\ 0 & 1} -\frac{2 \mathsf{T}_{\sigma_2 \sigma_3; \sigma_1 \sigma_4}}{N_f}\mathsf{R}( K, P).
\end{aligned}
\label{eq:etabeta2}
\end{equation}
Let us now use the tensors $\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} = \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} - \delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}$ and $\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} = \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} + \delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}$ and define
\begin{equation}
\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\{K_i\}} = \tilde{\lambda}^{\mathrm{I}; (+)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} + \tilde{\lambda}^{\mathrm{I}; (-)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\label{eq:spinseparation}
\end{equation}
following to Eq. \eqref{eq:ST}. Using this last equation together with the following Identities:
\begin{equation}
\begin{aligned}
\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\{K_i\}} \mathsf{S}^{\beta \alpha}_{\sigma_4 \sigma_3} = & 2\tilde{\lambda}^{\mathrm{I}; (+)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\\ \tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\{K_i\}} \mathsf{A}^{\beta \alpha}_{\sigma_4 \sigma_3} = & 2\tilde{\lambda}^{\mathrm{I}; (-)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\\ \delta_{\sigma_4 \sigma_1}\delta_{\sigma_3 \sigma_2} = & \frac{1}{2}\left(\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} + \mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}\right),
\\ \mathsf{T}_{\sigma_4 \beta; \sigma_3 \alpha}\mathsf{A}^{\sigma_1 \sigma_2}_{\beta \alpha} = & -2\left(1 + \frac{1}{N_c} \right)\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\\ \mathsf{T}_{\sigma_4 \beta; \sigma_3 \alpha}\mathsf{S}^{\sigma_1 \sigma_2}_{\beta \alpha} = & 2\left(1 - \frac{1}{N_c} \right)\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\end{aligned}
\label{eq:spinproj}
\end{equation}
we can write two equations from Eq. \eqref{eq:etabeta2}, one each spin channel. Moreover, let us separate the hot spot index matrix $\tilde{\lambda}$ into the $s$-wave and $d$-wave channels using the respective projectors
\begin{equation}
I = \pmqty{1 & 0 \\ 0 & 1}, \ P_s = \frac{1}{2}\pmqty{1 & 1 \\ 1 & 1}, \  P_d = \frac{1}{2}\pmqty{1 & -1 \\ -1 & 1},
\label{eq:waveproj}
\end{equation} 
where $P_s + P_d = I$ and $P_s - P_d = \spmqty{0 & 1 \\ 1 & 0}$. Therefore,
\begin{equation}
\tilde{\lambda}^{I;(\pm)}_{\spmqty{P & -P \\ K & -K}} = \tilde{\lambda}^{I;(\pm),(s)}_{\spmqty{P & -P \\ K & -K}}P_s + \tilde{\lambda}^{I;(\pm),(d)}_{\spmqty{P & -P \\ K & -K}}P_d.
\label{eq:waveseparation}
\end{equation}
In general
\begin{equation}
\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\{K_i\}} = \tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_s + \tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_s + \tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_d + \tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_d.
\label{eq:fullseparation}
\end{equation}
Let us define the following symbol 
\begin{equation}
1^{\spmqty{s \\ d}} = \left\lbrace \begin{matrix} 1, & \spmqty{s \\ d} = (s) \\ -1, & \spmqty{s \\ d} = (d) \end{matrix}\right.,
\label{eq:pmwavesymbol}
\end{equation}
and the following notation for the elements of $\mathsf{R}$
\begin{equation}
\mathsf{r}( K, P) = \frac{z (\hat{g}_{K, P})^2}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\frac{\Lambda_f^2}{\left(\Lambda_f + c \abs{K -P} + c \abs{\hat{v}_{K}K + \hat{v}_{P}P}\right)^2}.
\label{eq:Rsmallscaled}
\end{equation}
With the expressions \eqref{eq:spinseparation}-\eqref{eq:Rsmallscaled}, we can separate the matrix equation \eqref{eq:etabeta2} in four scalar equations, as follows:
\begin{equation}
\begin{aligned}
\frac{\partial }{\partial\ell}\tilde{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (\pm ),\spmqty{s \\ d}}_{\spmqty{P & -P \\ Q & -Q}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{P, Q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{P} \abs{P}}
\delta(P - Q) \right)
\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{Q & -Q \\ K & -K}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{Q,K})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_Q \abs{Q}}\delta(Q - K)\right)
\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(P-K) + 1^{\spmqty{s \\ d}}\frac{2}{N_f}\left(\frac{1}{N_c} \mp 1\right) \mathsf{r}(K, P).
\label{eq:betaallwavesscaled}
\end{aligned}
\end{equation}


%For the triplet channel:
%\begin{equation}
%\begin{aligned}
%\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{P & -P \\ K & -K}}
%\\ & -\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{P & -P \\ Q & -Q}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{P, Q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{P} \abs{P}}
%\delta(P - Q)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{Q & -Q \\ K & -K}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{Q,K})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_Q \abs{Q}}\delta(Q - K)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(P-K)\spmqty{1 & 0 \\ 0 & 1} -\frac{2}{N_f}\left(1-\frac{1}{N_c}\right)\mathsf{R}( K, P).
%\label{eq:betasym}
%\end{aligned}
%\end{equation}
%For the spin singlet channel:
%\begin{equation}
%\begin{aligned}
%\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{P & -P \\ K & -K}}
%\\ & -\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{P & -P \\ Q & -Q}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{P, Q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{P} \abs{P}}
%\delta(P - Q)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{Q & -Q \\ K & -K}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{Q,K})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_Q \abs{Q}}\delta(Q - K)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(P-K)\spmqty{1 & 0 \\ 0 & 1} + \frac{2}{N_f}\left(1+\frac{1}{N_c}\right)\mathsf{R}( K, P).
%\label{eq:betaantisym}
%\end{aligned}
%\end{equation}

To further approximate the last two equations, we reverse back to physical momentum, i.e. if $K$ and $P$ are rescaled momenta, and $k, p$ are physical momentum, then $K = e^{\ell}k$, $P = e^{\ell}p$ and
\begin{equation}
\begin{aligned}
\overline{\lambda}^{\mathrm{I}}_{\spmqty{p & -p \\ k & -k}} = & e^{\ell}\tilde{\lambda}^{\mathrm{I}}_{\spmqty{P & -P \\ K & -K}},
\\ g_{k,p} = & \hat{g}_{K,P}.
\end{aligned}
\label{eq:physicalchange}
\end{equation} 
Finally, $Q \to e^{\ell}q$ in the integrals. In physical momentum, Eq. \eqref{eq:fullseparation} still applies, so we can write \eqref{eq:betaallwavesscaled} directly in physical momentum as
% the beta functions are
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k)\spmqty{1 & 0 \\ 0 & 1} -\frac{2}{N_f}\left(1-\frac{1}{N_c}\right) e^{\ell}\mathsf{R}( k e^{\ell}, p e^{\ell}),
%\label{eq:betasymphysical1}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k)\spmqty{1 & 0 \\ 0 & 1} + \frac{2}{N_f}\left(1+\frac{1}{N_c}\right) e^{\ell}\mathsf{R}( k e^{\ell}, p e^{\ell}),
%\label{eq:betaantisymphysical1}
%\end{aligned}
%\end{equation}
%where the equations have been multiplied by $e^{\ell}$. Now, let us separate the hot spot index matrix $\tilde{\lambda}$ into the $s$-wave and $d$-wave channels using the respective projectors
%\begin{equation}
%P_s = \frac{1}{2}\pmqty{1 & 1 \\ 1 & 1}, \  P_d = \frac{1}{2}\pmqty{1 & -1 \\ -1 & 1},
%\end{equation} 
%where $P_s + P_d = \spmqty{1 & 0 \\ 0 & 1}$. Therefore,
%\begin{equation}
%\tilde{\lambda}^{I;(\pm)}_{\spmqty{p & -p \\ k & -k}} = \tilde{\lambda}^{I;(\pm),(s)}_{\spmqty{p & -p \\ k & -k}}P_s + \tilde{\lambda}^{I;(\pm),(d)}_{\spmqty{p & -p \\ k & -k}}P_d.
%\end{equation}
%In the last equation, $\tilde{\lambda}^{I;(\pm),(s)}_{\spmqty{p & -p \\ k & -k}}$ and $\tilde{\lambda}^{I;(\pm),(d)}_{\spmqty{p & -p \\ k & -k}}$ are scalars with respect to the hot spot super-indices $(15)$ and $(48)$. Additionally, from Eq. \eqref{eq:newRel}, let us separate the coefficient containing the propagator and Yukawa coupling $g$, which we call $\tilde{r}$, from the hot spot matrix explicitly by writing
%\begin{equation}
%\mathsf{R}( k, p) = \tilde{r}(\ell; k, p)\spmqty{0 & 1 \\ 1 & 0} = \tilde{r}(\ell; k, p)(P_s - P_d).
%\end{equation}
%In the basis $P_s, P_d$, we have four beta function equations. For the triplet channel we have two equations, the $s$-wave beta function is
%\begin{subequations}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) -\frac{2}{N_f}\left(1-\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}),
%\label{eq:betasymswave}
%\end{aligned}
%\end{equation}
%and the $d$-wave equation is
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\spmqty{p & -p \\ k & -k}} =  & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) +\frac{2}{N_f}\left(1-\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}).
%\label{eq:betasymdwave}
%\end{aligned}
%\end{equation}
%\end{subequations}
%For the singlet channel we also have two equations, the $s$-wave beta function is
%\begin{subequations}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) +\frac{2}{N_f}\left(1+\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}),
%\label{eq:betaantisymswave}
%\end{aligned}
%\end{equation}
%and the $d$-wave equation is
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) - \frac{2}{N_f}\left(1+\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}).
%\label{eq:betaantisymdwave}
%\end{aligned}
%\end{equation}
%\end{subequations}
%We can write all these equations in one simple expression. Let us define the following symbol 
%\begin{equation}
%1^{\spmqty{s \\ d}} = \left\lbrace \begin{matrix} 1, & \spmqty{s \\ d} = s \\ -1, & \spmqty{s \\ d} = d \end{matrix}\right.
%\end{equation}
\begin{equation}
\begin{aligned}
\frac{\dd }{\dd\ell}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm ),\spmqty{s \\ d}}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
\delta(p - q) \right)
\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q - k)\right)
\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) + 1^{\spmqty{s \\ d}}\frac{2}{N_f}\left(\frac{1}{N_c} \mp 1\right) \tilde{r}(\ell; k, p),
\label{eq:betaallwaves}
\end{aligned}
\end{equation}
where
\begin{equation}
\tilde{r}(\ell; k, p) = \frac{ z g_{k, p}^2}{\sqrt{V_{F,k}V_{F,p}}}
 \frac{\Lambda_f^2  e^{-\ell}}{\left(\Lambda_f e^{-\ell} + c \abs{k-p} + c \abs{v_{k}k + v_{p}p}\right)^2},
\label{eq:Rsmallphys}
\end{equation}
analogous to Eq. \eqref{eq:Rsmallscaled}.













\section{More details in the derivation of \ffc beta functionals}

Let us now use the tensors $\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} = \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} - \delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}$ and $\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} = \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} + \delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4}$ and define
\begin{equation}
\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\{K_i\}} = \tilde{\lambda}^{\mathrm{I}; (+)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} + \tilde{\lambda}^{\mathrm{I}; (-)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\label{eq:spinseparation}
\end{equation}
following to Eq. \eqref{eq:ST}. Using this last equation together with the following Identities:
\begin{equation}
\begin{aligned}
\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\{K_i\}} \mathsf{S}^{\beta \alpha}_{\sigma_4 \sigma_3} = & 2\tilde{\lambda}^{\mathrm{I}; (+)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\\ \tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\{K_i\}} \mathsf{A}^{\beta \alpha}_{\sigma_4 \sigma_3} = & 2\tilde{\lambda}^{\mathrm{I}; (-)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\\ \delta_{\sigma_4 \sigma_1}\delta_{\sigma_3 \sigma_2} = & \frac{1}{2}\left(\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3} + \mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}\right),
\\ \mathsf{T}_{\sigma_4 \beta; \sigma_3 \alpha}\mathsf{A}^{\sigma_1 \sigma_2}_{\beta \alpha} = & -2\left(1 + \frac{1}{N_c} \right)\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\\ \mathsf{T}_{\sigma_4 \beta; \sigma_3 \alpha}\mathsf{S}^{\sigma_1 \sigma_2}_{\beta \alpha} = & 2\left(1 - \frac{1}{N_c} \right)\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3},
\end{aligned}
\label{eq:spinproj}
\end{equation}
we can write two equations from Eq. \eqref{eq:etabeta2}, one each spin channel. Moreover, let us separate the hot spot index matrix $\tilde{\lambda}$ into the $s$-wave and $d$-wave channels using the respective projectors
\begin{equation}
I = \pmqty{1 & 0 \\ 0 & 1}, \ P_s = \frac{1}{2}\pmqty{1 & 1 \\ 1 & 1}, \  P_d = \frac{1}{2}\pmqty{1 & -1 \\ -1 & 1},
\label{eq:waveproj}
\end{equation} 
where $P_s + P_d = I$ and $P_s - P_d = \spmqty{0 & 1 \\ 1 & 0}$. Therefore,
\begin{equation}
\tilde{\lambda}^{I;(\pm)}_{\spmqty{P & -P \\ K & -K}} = \tilde{\lambda}^{I;(\pm),(s)}_{\spmqty{P & -P \\ K & -K}}P_s + \tilde{\lambda}^{I;(\pm),(d)}_{\spmqty{P & -P \\ K & -K}}P_d.
\label{eq:waveseparation}
\end{equation}
In general
\begin{equation}
\tilde{\lambda}^{\mathrm{I}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\{K_i\}} = \tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_s + \tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_s + \tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\{K_i\}}\mathsf{S}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_d + \tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\{K_i\}}\mathsf{A}^{\sigma_1 \sigma_2}_{\sigma_4 \sigma_3}P_d.
\label{eq:fullseparation}
\end{equation}
Let us define the following symbol 
\begin{equation}
1^{\spmqty{s \\ d}} = \left\lbrace \begin{matrix} 1, & \spmqty{s \\ d} = (s) \\ -1, & \spmqty{s \\ d} = (d) \end{matrix}\right.,
\label{eq:pmwavesymbol}
\end{equation}
and the following notation for the elements of $\mathsf{R}$
\begin{equation}
\mathsf{r}( K, P) = \frac{z (\hat{g}_{K, P})^2}{\sqrt{\hat{V}_{F,K}\hat{V}_{F,P}}}\frac{\Lambda_f^2}{\left(\Lambda_f + c \abs{K -P} + c \abs{\hat{v}_{K}K + \hat{v}_{P}P}\right)^2}.
\label{eq:Rsmallscaled}
\end{equation}
With the expressions \eqref{eq:spinseparation}-\eqref{eq:Rsmallscaled}, we can separate the matrix equation \eqref{eq:etabeta2} in four scalar equations, as follows:
\begin{equation}
\begin{aligned}
\frac{\partial }{\partial\ell}\tilde{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{P & -P \\ K & -K}}
\\ & -\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (\pm ),\spmqty{s \\ d}}_{\spmqty{P & -P \\ Q & -Q}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{P, Q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{P} \abs{P}}
\delta(P - Q) \right)
\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{Q & -Q \\ K & -K}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{Q,K})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_Q \abs{Q}}\delta(Q - K)\right)
\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(P-K) + 1^{\spmqty{s \\ d}}\frac{2}{N_f}\left(\frac{1}{N_c} \mp 1\right) \mathsf{r}(K, P).
\label{eq:betaallwavesscaled}
\end{aligned}
\end{equation}


%For the triplet channel:
%\begin{equation}
%\begin{aligned}
%\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{P & -P \\ K & -K}}
%\\ & -\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{P & -P \\ Q & -Q}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{P, Q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{P} \abs{P}}
%\delta(P - Q)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{Q & -Q \\ K & -K}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{Q,K})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_Q \abs{Q}}\delta(Q - K)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(P-K)\spmqty{1 & 0 \\ 0 & 1} -\frac{2}{N_f}\left(1-\frac{1}{N_c}\right)\mathsf{R}( K, P).
%\label{eq:betasym}
%\end{aligned}
%\end{equation}
%For the spin singlet channel:
%\begin{equation}
%\begin{aligned}
%\frac{\partial}{\partial\ell}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{P & -P \\ K & -K}} = & -\left(1 + K\frac{\partial}{\partial K} + P\frac{\partial}{\partial P} \right)\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{P & -P \\ K & -K}}
%\\ & -\int \frac{\dd Q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{P & -P \\ Q & -Q}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{P, Q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{P} \abs{P}}
%\delta(P - Q)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{Q & -Q \\ K & -K}} + \sqrt{2\pi}\Lambda_f \frac{(\hat{g}_{Q,K})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_Q \abs{Q}}\delta(Q - K)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c \hat{v}_{K} \abs{K}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(\hat{g}_{K,K})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(P-K)\spmqty{1 & 0 \\ 0 & 1} + \frac{2}{N_f}\left(1+\frac{1}{N_c}\right)\mathsf{R}( K, P).
%\label{eq:betaantisym}
%\end{aligned}
%\end{equation}

To further approximate the last two equations, we reverse back to physical momentum, i.e. if $K$ and $P$ are rescaled momenta, and $k, p$ are physical momentum, then $K = e^{\ell}k$, $P = e^{\ell}p$ and
\begin{equation}
\begin{aligned}
\overline{\lambda}^{\mathrm{I}}_{\spmqty{p & -p \\ k & -k}} = & e^{\ell}\tilde{\lambda}^{\mathrm{I}}_{\spmqty{P & -P \\ K & -K}},
\\ g_{k,p} = & \hat{g}_{K,P}.
\end{aligned}
\label{eq:physicalchange}
\end{equation} 
Finally, $Q \to e^{\ell}q$ in the integrals. In physical momentum, Eq. \eqref{eq:fullseparation} still applies, so we can write \eqref{eq:betaallwavesscaled} directly in physical momentum as
% the beta functions are
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k)\spmqty{1 & 0 \\ 0 & 1} -\frac{2}{N_f}\left(1-\frac{1}{N_c}\right) e^{\ell}\mathsf{R}( k e^{\ell}, p e^{\ell}),
%\label{eq:betasymphysical1}
%\end{aligned}
%\end{equation}
%and
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\spmqty{1 & 0 \\ 0 & 1} \right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k)\spmqty{1 & 0 \\ 0 & 1} + \frac{2}{N_f}\left(1+\frac{1}{N_c}\right) e^{\ell}\mathsf{R}( k e^{\ell}, p e^{\ell}),
%\label{eq:betaantisymphysical1}
%\end{aligned}
%\end{equation}
%where the equations have been multiplied by $e^{\ell}$. Now, let us separate the hot spot index matrix $\tilde{\lambda}$ into the $s$-wave and $d$-wave channels using the respective projectors
%\begin{equation}
%P_s = \frac{1}{2}\pmqty{1 & 1 \\ 1 & 1}, \  P_d = \frac{1}{2}\pmqty{1 & -1 \\ -1 & 1},
%\end{equation} 
%where $P_s + P_d = \spmqty{1 & 0 \\ 0 & 1}$. Therefore,
%\begin{equation}
%\tilde{\lambda}^{I;(\pm)}_{\spmqty{p & -p \\ k & -k}} = \tilde{\lambda}^{I;(\pm),(s)}_{\spmqty{p & -p \\ k & -k}}P_s + \tilde{\lambda}^{I;(\pm),(d)}_{\spmqty{p & -p \\ k & -k}}P_d.
%\end{equation}
%In the last equation, $\tilde{\lambda}^{I;(\pm),(s)}_{\spmqty{p & -p \\ k & -k}}$ and $\tilde{\lambda}^{I;(\pm),(d)}_{\spmqty{p & -p \\ k & -k}}$ are scalars with respect to the hot spot super-indices $(15)$ and $(48)$. Additionally, from Eq. \eqref{eq:newRel}, let us separate the coefficient containing the propagator and Yukawa coupling $g$, which we call $\tilde{r}$, from the hot spot matrix explicitly by writing
%\begin{equation}
%\mathsf{R}( k, p) = \tilde{r}(\ell; k, p)\spmqty{0 & 1 \\ 1 & 0} = \tilde{r}(\ell; k, p)(P_s - P_d).
%\end{equation}
%In the basis $P_s, P_d$, we have four beta function equations. For the triplet channel we have two equations, the $s$-wave beta function is
%\begin{subequations}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(s)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) -\frac{2}{N_f}\left(1-\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}),
%\label{eq:betasymswave}
%\end{aligned}
%\end{equation}
%and the $d$-wave equation is
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\spmqty{p & -p \\ k & -k}} =  & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (+),(d)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) +\frac{2}{N_f}\left(1-\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}).
%\label{eq:betasymdwave}
%\end{aligned}
%\end{equation}
%\end{subequations}
%For the singlet channel we also have two equations, the $s$-wave beta function is
%\begin{subequations}
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(s)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) +\frac{2}{N_f}\left(1+\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}),
%\label{eq:betaantisymswave}
%\end{aligned}
%\end{equation}
%and the $d$-wave equation is
%\begin{equation}
%\begin{aligned}
%\frac{\dd }{\dd\ell}\tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q_x}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
%\delta(p - q_x) \right)
%\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\tilde{\lambda}^{\mathrm{I}; (-),(d)}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q_x - k)\right)
%\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) - \frac{2}{N_f}\left(1+\frac{1}{N_c}\right) e^{\ell}\tilde{r}(\ell; k e^{\ell}, p e^{\ell}).
%\label{eq:betaantisymdwave}
%\end{aligned}
%\end{equation}
%\end{subequations}
%We can write all these equations in one simple expression. Let us define the following symbol 
%\begin{equation}
%1^{\spmqty{s \\ d}} = \left\lbrace \begin{matrix} 1, & \spmqty{s \\ d} = s \\ -1, & \spmqty{s \\ d} = d \end{matrix}\right.
%\end{equation}
\begin{equation}
\begin{aligned}
\frac{\dd }{\dd\ell}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{p & -p \\ k & -k}} = & -\int \frac{\dd q}{2\pi\Lambda_f}\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm ),\spmqty{s \\ d}}_{\spmqty{p & -p \\ q & -q}} + \sqrt{2\pi}\Lambda_f \frac{(g_{p, q})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_{p} \abs{p}e^{\ell}}
\delta(p - q) \right)
\\ & \hspace{2cm}\times\left( \frac{1}{\sqrt{2\pi}}\overline{\lambda}^{\mathrm{I}; (\pm),\spmqty{s \\ d}}_{\spmqty{q & -q \\ k & -k}} + \sqrt{2\pi}\Lambda_f \frac{(g_{q,k})^2(N_c^2 -1)}{\pi c N_c N_f}\frac{\Lambda_f}{\Lambda_f + 2 c v_q \abs{q_x}e^{\ell}}\delta(q - k)\right)
\\ & + \Lambda_f \left[\frac{\Lambda_f}{\Lambda_f + 2 c v_{k} \abs{k}e^{\ell}}\right]^2 \frac{\left(N_c^2 - 1\right)^2(g_{k,k})^4}{\pi^2 c^2 N_c^2 N_f^2}\delta(p-k) + 1^{\spmqty{s \\ d}}\frac{2}{N_f}\left(\frac{1}{N_c} \mp 1\right) \tilde{r}(\ell; k, p),
\label{eq:betaallwaves}
\end{aligned}
\end{equation}
where
\begin{equation}
\tilde{r}(\ell; k, p) = \frac{ z g_{k, p}^2}{\sqrt{V_{F,k}V_{F,p}}}
 \frac{\Lambda_f^2  e^{-\ell}}{\left(\Lambda_f e^{-\ell} + c \abs{k-p} + c \abs{v_{k}k + v_{p}p}\right)^2},
\label{eq:Rsmallphys}
\end{equation}
analogous to Eq. \eqref{eq:Rsmallscaled}.







\section{hot spot beta functions}


{\bf [SL : move this to appendix; rewrite using $T$ tensor]}
The beta functional at the origin for momentum $\spmqty{0 & 0 \\ 0 & 0}$ is
\begin{equation*}
\begin{aligned}
& \beta^{(\lambda);\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3(z-1) + 4\eta^{(\psi)}_{0} \right) \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} 
\\ & - \frac{1}{\pi N_f}\int \dd\rho(q) \mathsf{D}(0;q) 
\left\lbrace \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} +  \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{0 & 0 \\ q & -q}} 
% \right. \\ &  
-\frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ q & -q}} \right.
\\ &
\left. - \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\delta_{\sigma_2 \sigma_4} + \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}}\delta_{\sigma_1 \sigma_3} \right) 
+ \frac{1}{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & q \\ q & 0}} 
%\right. \\ & \left. \left. 
+ \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & 0 \\ 0 & q}} \right) \right\rbrace  \\&
 + \frac{v_0}{2\pi c N_f}\left[ \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)
 %\right. \\ & \left. 
 - \frac{1}{N_c} \left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\right) \right]  \\&
 + \left( 2 \text{Li}_2\left(-\frac{1}{2}\right) + \pi^2 + \log^2(2) \right)\frac{v_0^2}{4 N_f^2 c}\left( \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} - N_c \delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} \right)
\\ & + 
\frac{1}{4 \pi } \int \dd\rho(q) \sum_{\alpha, \beta = 1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\ q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\ q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} \right.
\\ & \left. - \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}} - \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}}\right).
\end{aligned}
\end{equation*}
The last term in this expression corresponds to the source term and represents a total subtraction of the quantum effective action. Since this term is a constant, not depending on any IR divergences, and we are limiting ourselves to a minimal subtraction scheme we drop this term. The final answer is then
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{1 & 5 \\ 1 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3(z-1) + 4\eta^{(\psi)}_{0} \right) \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} 
\\ & 
- \frac{1}{\pi N_f}\int \dd\rho(q) \mathsf{D}(0;q) 
\left\lbrace 
\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} 
%\\ &
 - \frac{1}{N_c}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} +  \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{0 & 0 \\ q & -q}}  
%\right. \\ &  
-\frac{1}{N_c}\lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ q & -q}} \right.
\\& 
\left.
- \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\delta_{\sigma_2 \sigma_4} + \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}}\delta_{\sigma_1 \sigma_3} \right) 
+ \frac{1}{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & q \\ q & 0}} 
%\right.\\ & \left. \left. 
+ \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & 0 \\ 0 & q}} \right) \right\rbrace 
\\&
 + \frac{v_0}{2\pi c N_f}\left[ \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)
%\right.\\ & \left. 
- \frac{1}{N_c} \left( \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} + \lambda^{\spmqty{1 & 8 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\right) \right]
\\ & + \frac{1}{4 \pi} \int \dd\rho(q) \sum_{\alpha, \beta = 1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\ q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\ q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} \right.
\\ & \left. - \lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}} - \lambda^{\spmqty{1 & 8 \\ 4 & 5}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}}\right).
\end{aligned}
\end{equation}
%\end{enumerate}

The beta functional for 
$\lambda^{\spmqty{1 & 5 \\ 1 & 5}}$
depends on 
$\lambda^{\spmqty{4 & 8 \\ 1 & 5}}$,
$\lambda^{\spmqty{4 & 5 \\ 8 & 1}}$ and
$\lambda^{\spmqty{4 & 5 \\ 4 & 5}}$.
To have a closed set of equations,
we need the beta functionals for those coupling functions.
Below, we list the beta functionals for each of
$\lambda^{\spmqty{4 & 8 \\ 1 & 5}}$,
$\lambda^{\spmqty{4 & 5 \\ 8 & 1}}$ and
$\lambda^{\spmqty{4 & 5 \\ 4 & 5}}$.



\paragraph{The beta functional for $\lambda^{\spmqty{4 & 8 \\ 1 & 5}}$}
{\bf [SL : move beta functionals at hot spots to appendix; rewrite using $T$ tensor]}

For $\lambda^{\spmqty{4 & 8 \\ 1 & 5}}$,
quantum corrections are present 
only within the PP-plane because
only the pairs of $(1,5)$ and $(4,8)$
are nested in the particle-particle channel. 

\begin{enumerate}



%In terms of the logarithmic length scale
%\begin{equation}
%\begin{aligned}
%\frac{\partial}{\partial \ell}\hat{\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}} = & -K\frac{\partial}{\partial K}\hat{\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}-P\frac{\partial}{\partial P}\hat{\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
%\\ & -\left( 1 + 3(z-1) + \hat{\eta}^{(\psi)}_{P} + \hat{\eta}^{(\psi)}_{-P} + \hat{\eta}^{(\psi)}_{K} + \hat{\eta}^{(\psi)}_{-K} \right)\hat{\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -P \\ K & -K}}
%\\ & - \frac{1}{\pi}\int \dd \rho(Q)\sum_{\beta, \alpha = 1}^{N_c} \left\lbrace -\frac{1}{2 N_f}\left[\mathsf{D}(Q;P)\mathsf{T}_{\sigma_2 \alpha ; \sigma_1 \beta} \hat{\lambda}^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} \right. \right. 
%\\ & \left. + \mathsf{D}(Q;K)\mathsf{T}_{\sigma_3 \alpha ; \sigma_4 \beta} \hat{\lambda}^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}}\right]
%\\ &\left. + \frac{1}{4}\left(\hat{\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}}\hat{\lambda}^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} + \hat{\lambda}^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{P & -P \\ Q & -Q}}\hat{\lambda}^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{Q & -Q \\ K & -K}} \right)\right\rbrace.
%\end{aligned}
%\label{eq:betalambda2PP}
%\end{equation}

\item 
The beta functional at momentum $\spmqty{0 & 0 \\ 0 & 0}$ is
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3(z-1) + 4\eta^{(\psi)}_{0} \right) \lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & +\frac{v_0}{4\pi N_f}\frac{\pi v_0 + 2c(1+v_0)\log(c(1+1/v_0))}{c^2(1+v_0)^2+v_0^2}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 8 \\ 4 & 5} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 5 \\ 1 & 8} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{4 & 5 \\ 1 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\right]
\\ & \frac{1}{\pi N_f} \int \dd\rho(q)  \mathsf{D}(0;q)  \left[ \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_2 & \sigma_1 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_3 & \sigma_4}}_{\spmqty{0 & 0 \\ q & -q}}  - \frac{1}{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} + \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ q & -q}} \right) \right]
\\ & + \frac{1}{4 \pi} \int  \dd\rho(q) \sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\ q & -q}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \beta & \alpha}}_{\spmqty{0 & 0 \\ q & -q}}\lambda^{\spmqty{4 & 8 \\ 1 & 5}; \spmqty{\beta & \alpha \\ \sigma_4 & \sigma_3}}_{\spmqty{q & -q \\ 0 & 0}} \right).
\end{aligned}
\end{equation}

\end{enumerate}

\paragraph{The beta functional for $\lambda^{\spmqty{4 & 5 \\ 1 & 8}}$}


This is the particle-hole counterpart 
of $\lambda^{\spmqty{4 & 8 \\ 1 & 5}}$.
For $\lambda^{\spmqty{4 & 5 \\ 1 & 8}}$,
quantum corrections are present 
only within the PH-plane because
only the pairs of $(1,5)$ and $(4,8)$
are nested in the particle-hole channel. 

\begin{enumerate}


%In terms of the logarithmic length scale
%\begin{equation}
%\begin{aligned}
%\frac{\partial}{\partial \ell}\hat{\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & K \\ K & P}} = & -K\frac{\partial}{\partial K}\hat{\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & K \\ K & P}}-P\frac{\partial}{\partial P}\hat{\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & -K \\ K & P}}
%\\ & -\left( 1 + 3(z-1) + 2\hat{\eta}^{(\psi)}_{P} + 2\hat{\eta}^{(\psi)}_{K} \right)\hat{\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{P & K \\ K & P}}
%\\ & - \frac{1}{\pi}\int \dd \rho(Q)\sum_{\beta, \alpha = 1}^{N_c} \left\lbrace \frac{1}{2 N_f}\left[\mathsf{D}(Q;K)\mathsf{T}_{\alpha \sigma_2 ; \sigma_4 \beta} \hat{\lambda}^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{P & Q \\ Q & P}} \right. \right.
%\\ & \left. + \mathsf{D}(Q;P)\mathsf{T}_{\beta \sigma_1 ; \sigma_3 \alpha} \hat{\lambda}^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{Q & K \\ K & Q}}\right]
%\\ &\left. - \frac{1}{4}\sum_{\alpha, \beta = 1}^{N_c}\left(\hat{\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{P & Q \\ Q & P}}\hat{\lambda}^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{Q & K \\ K & Q}} + \hat{\lambda}^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{P & Q \\ Q & P}}\hat{\lambda}^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{Q & K \\ K & Q}} \right)\right\rbrace.
%\end{aligned}
%\label{eq:betalambda3PH}
%\end{equation}

\item 
{\bf [SL : move this to appendix; rewrite using $T$ tensor]}
The beta functional at momentum $\spmqty{0 & 0 \\ 0 & 0}$ is
\begin{equation}
\begin{aligned}
& \beta^{(\lambda);\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = \left( 1 + 3(z-1) + 4\eta^{(\psi)}_{0} \right) \lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & + \frac{v_0}{4\pi N_f}\frac{\pi v_0 + 2c(1+v_0)\log(c(1+1/v_0))}{c^2(1+v_0)^2+v_0^2}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 4 & 8} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 8 \\ 1 & 5} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{4 & 8 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} \right]
\\ & +\frac{1}{\pi N_f} \int \dd\rho(q) 
\mathsf{D}(0;q) 
\left[ \sum_{\alpha = 1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}}\delta_{\sigma_1 \sigma_3} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \alpha & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\delta_{\sigma_2 \sigma_4}  \right) 
%\right. \\ & \left. 
-\frac{1}{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{q & 0 \\ 0 & q}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & q \\ q & 0}} \right) \right]
\\ & - \frac{1}{4 \pi} \int  \dd\rho(q) \sum_{\alpha, \beta = 1}^{N_c}\left(\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\lambda^{\spmqty{1 & 5 \\ 1 & 5}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}} + \lambda^{\spmqty{4 & 8 \\ 4 & 8}; \spmqty{\sigma_1 & \alpha \\ \beta & \sigma_3}}_{\spmqty{0 & q \\ q & 0}}\lambda^{\spmqty{4 & 5 \\ 1 & 8}; \spmqty{\beta & \sigma_2 \\ \sigma_4 & \alpha}}_{\spmqty{q & 0 \\ 0 & q}} \right).
\end{aligned}
\end{equation}

\end{enumerate}

\paragraph{The beta functional for $\lambda^{\spmqty{4 & 5 \\ 4 & 5}}$}

For  $\lambda^{\spmqty{4 & 5 \\ 4 & 5}}$,
quantum corrections are present only 
when external momenta are zero.
In a total subtraction scheme, the beta functionals would be written as
\begin{equation*}
\begin{aligned}
\beta^{(\lambda);\spmqty{4 & 5 \\ 4 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = & \left( 1 + 3(z-1) + 4\eta^{(\psi)}_{0} \right) \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & - \frac{v_0}{2\pi c(1+v_0) N_f}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} \right]
\\ & + \left( \frac{\pi^2}{4} + \log\left(\frac{27}{4}\right) \right)\frac{v_0^2}{2 N_f^2 c}\left( N_c\delta_{\sigma_1 \sigma_3}\delta_{\sigma_2 \sigma_4} - \delta_{\sigma_1 \sigma_4}\delta_{\sigma_2 \sigma_3} \right).
\end{aligned}
\end{equation*}
In the minimal subtraction scheme,
we drop those contributions in the zero-dimensional manifold
to obtain
\begin{equation}
\begin{aligned}
\beta^{(\lambda);\spmqty{4 & 5 \\ 4 & 5};\spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} = & \left( 1 + 3(z-1) + 4\eta^{(\psi)}_{0} \right) \lambda^{\spmqty{4 & 5 \\ 4 & 5}; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}
\\ & - \frac{v_0}{2\pi c(1+v_0) N_f}\left[ \sum_{\alpha=1}^{N_c}\left( \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\alpha & \sigma_2 \\ \alpha & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_1 \sigma_4} + \lambda^{\spmqty{4 & 8 \\ 4 & 8} ; \spmqty{\sigma_1 & \alpha \\ \sigma_4 & \alpha}}_{\spmqty{0 & 0 \\ 0 & 0}}\delta_{\sigma_2 \sigma_3} \right)  - \frac{2}{N_c} \lambda^{\spmqty{1 & 5 \\ 1 & 5} ; \spmqty{\sigma_1 & \sigma_2 \\ \sigma_4 & \sigma_3}}_{\spmqty{0 & 0 \\ 0 & 0}} \right].
\end{aligned}
\end{equation}



==> single.tex <==







\newcommand{\mcTnfl}{\mc T_{\scriptscriptstyle{\textrm{NFL}}}}
\newcommand{\mcTfl}{\mc T_{\scriptscriptstyle{\textrm{FL}}}}




\section{Single-particle properties}







\subsection{Beta functions}

To the leading order in $v$,
we need to include the one-loop vertex correction,
and the one-loop and the two-loop corrections
for the fermion self-energy.
The counter terms 
to the fermion kinetic term
and the cubic coupling
obtained in the adiabatic limit
%in \eq{eq:CTAction}
are given by (see Appendix~\ref{app:QC} for derivation)
%
%Here we collect the counter terms 
%computed in
%\ref{A1Lashu,eq:A21L,eq:A31L,eqA12L,eqA22L,eqA32L,eqA41L}:
\begin{align}
A^{(1)}(k_N)
&=-\frac{N_c^2-1}{\pi^2 N_cN_f} \FR{g_k^2}{cV_{F,k}}
%\log\left( \FR{c\Lambda_b}{\mu+2v_kc|k_N|} \right)
\log\left( \FR{c\Lambda_b}{\mathscr{H}_1( \mu, 2v_kc|k_N|)} \right)
\nn
%A^{(1);2\mathrm{L}}_{N}(k_{N}) &=  
&-\frac{g_k^4(N_c^2-1)}{2\pi^4 c^2V_{F,k}^2N_c^2N_f^2}\log\left(\frac{v_kV_{F,k}}{c}\right)^2
\log\left(\frac{\Lambda_f}{\mathscr{H}_1(\mu,4V_{F,k}v_k|k_{N}|)}\right),
\nn
A^{(2)}_{N}(k_{N}) &=   \frac{2g_k^2(N_c^2-1)}{\pi^3 V_{F,k} N_cN_f} \log\left(\frac{V_{F,k}}{c}\right)\log\left(\frac{\Lambda_f}{\mathscr{H}_1(|\mu|,2 v_k c |k_{N}|)}\right)\nn
%A^{(2);2L}(k_N)
%&= 
&+\frac{3g_k^4(N_c^2-1)}{2\pi^4 c^2V_{F,k}^2N_c^2N_f^2}
\log\PFR{V_{F,k} v_k}{c}^2
\log\left(\frac{\Lambda_f}{\mathscr{H}_1(\mu,4V_{F,k}v_k|k_N|)}\right),
\nn
A^{(3)}_{N}(k_{N}) &= - \frac{2g_k^2(N_c^2-1)}{\pi^3 V_{F,k} N_cN_f} \log\left(\frac{V_{F,k}}{c}\right)\log\left(\frac{\Lambda_f}{\mathscr{H}_1(\mu, 2 v_k c |k_{N}|)}\right)
\nn
%\label{eqA32L}
%A^{(3);2L}(k_N)
%&= 
& -\frac{g_k^4(N_c^2-1)}{2\pi^4 c^2V_{F,k}^2N_c^2N_f^2}
\log\PFR{V_{F,k} v_k}{c}^2
\log\left(\frac{\Lambda_f}{\mathscr{H}_1(\mu,4V_{F,k}v_k|k_N|)}\right),
\nn
A^{(4)}_{N}(k'_{N},k_{{N}})
&=-\frac{g_kg_{k'}}{2\pi^2cN_cN_{f}}
\log\left(\frac{2c}{V_{F,k}v_k+V_{F,k'}v_{k'}}\right)\nonumber\\
&\;\;\times\left[\frac{1}{V_{F,k}}+\frac{1}{V_{F,k'}}\right]\log\left(\frac{\Lambda_f}
{\mathscr{H}_3(\mu,2v_{k'}c|k'_{N}|,2v_kc|k_{N}|,|V_{F,k'}v_{k'}k'_N+V_{F,k}v_kk_N|)}\right).
\label{eq:allcounterterms}
\end{align}
Here $g_k\equiv g_{k,k}$.
 $\mathscr{H}_i(x_1,k_2,..,x_{i+1})$'s 
represent smooth crossover functions that satisfy
\bqa
\mathscr{H}_i(x_1,k_2,..,x_{i+1})
\approx |x_j| ~~~
\mbox{ if $|x_j| \gg |x_1|,..,|x_{j-1}|,|x_{j+1}|,..,|x_i|$ }.
\label{eq:Hi}
\eqa
For example, the counter term that fully cancels 
the imaginary part of the one-loop fermion self-energy is  
\bqa
\mathscr{H}_1( x_1, x_2 ) = |x_1| + |x_2|.
\label{eq:H0}
\eqa
However, the specific form of  
$\mathscr{H}_i$ is not important
as far as the counter term removes all UV and IR divergences
in physical observables.
Choosing different $\mathscr{H}_i$ 
amounts to imposing a different set of 
renormalization conditions 
by modifying the finite parts, $\mathscr{F}_i$ 
in Eqs. (\ref{eq:RG1})-(\ref{eq:RG5}).
%A simple choice that satisfies \eq{eq:Hi} is
%$ \mathscr{H}_i(x_1,k_2,..,x_{i+1})
%= \sqrt{ \sum_i  x_j^2 }$.
%For $\mathscr{H}_i$ with $i \geq 1$, 
%we don't need to specify the precise crossover functions. 
%
$A^{(i)}(k)$ for $i=1,2,3$ are the counter terms
for the kinetic term of the electron at momentum $k$ away from the hot spots
along the Fermi surface.
$A^{(4)}(k',k)$ is the counter term for the 
cubic vertex that describes the scattering of electron
from momentum $k$ near hot spot $\bar N$
to momentum $k'$ near hot spot $N$.
In general, the quantum corrections are 
functionals of the coupling functions.
However, $A^{(i)}(k)$ for $i=1,2,3$ depend only on 
the coupling functions at momentum $k$
if the adiabaticity is satisfied, 
that is, the coupling functions at energy $\mu$
do not change appreciably as a function of 
the momentum along the Fermi surface   
over the momentum that is order of $\mu$.
Here, we first assume that the coupling functions satisfy adiabaticity, 
and show that the solution of the beta functionals
obtained under the assumption of adiabaticity
 indeed satisfy the adiabaticity.
Similarly, $A^{(4)}(k',k)$ depends only on the coupling functions 
that are defined at $k$ and $k'$
if adiabaticity is satisfied.
%
Each counter term is proportional to
\bqa
\log
\left[
\frac{\Lambda_f}{\mathscr{H}_i( \mu, \Delta_1,..,\Delta_i)} 
\right],
\label{eq:loglhi}
\eqa
where $\mu$ is the energy scale
at which the RG condition is imposed,
and $\Delta_i$ represents crossover energy scales 
that depend on external momenta.
If $\mu$ is much greater than all $\Delta_i$'s,
\eq{eq:loglhi} becomes $\log \left( \frac{\Lambda_f}{\mu} \right)$,
and the quantum correction gives rise to 
the logarithmic flow of the coupling functions as the energy is lowered.
If $\mu$ becomes much smaller than any of $\Delta_i$,
the quantum correction becomes independent of $\mu$,
and no longer contributes to the flow of coupling functions. 
Roughly speaking, the contribution to the beta function 
turns off below the energy scale
which is given by the largest of $\Delta_i$'s.
Since quantum corrections turn off at different energy scales
at different points on the Fermi surface,
the renormalized coupling functions acquire momentum dependence
at low energies
even if one starts with momentum independent coupling functions
at the UV cutoff scale.








%The $\ellonek,\elltwok$ and $\ellthreekkp$ 
%represent the logarithmic length scales over which 
%each of the quantum corrections turn off.
%They are determined from the following self-consistent equations,
%\begin{align}
%       \label{appEnCross1}
%       %%  E_1(k) \equiv 
%       \Lambda_f e^{-\ellonek} &= 2 V_{F}(x;\ellonek) v(x;\ellonek) x\\
%       \label{appEnCross2} 
%       %%E_2(k) \equiv 
%       \Lambda_f e^{-\elltwok} &= 2 v(k; \elltwok) c(\elltwok) k\\
%       \label{appEnCross3} 
%       %%E_3(k,k') \equiv 
%       \Lambda_f e^{-\ellthreekkp} &= 
%       \max\left(
%               2\FR{|v(x;\ellthreekkp)x+v(x'; \ellthreekkp)x'|}{V_{F}(x;\ellthreekkp)^{-1}+V_{F}(x';\ellthreekkp)^{-1}},
%               2v(x;\ellthreekkp)c(\ellthreekkp) x,
%               2v(x';\ellthreekkp)c(\ellthreekkp) x'
%       \right)
%\end{align}








\begin{figure*}
    \centering
    \includegraphics[scale=1]{./Figures/crossover_scales_SCINF.pdf}
    \caption{
        Crossover scales energy scales in the case in which $\ell_{\mathrm{SC}}=\infty$. The shaded regions are where the quantum corrections have nonzero support as a function of energy and momentum. 
{\bf[ Revise the figure so that the notations are compatible with those in the text]}
    }
    \label{fig:crossover}
\end{figure*}




From 
Eqs. (\ref{eq:newZ1})
-
(\ref{eq:newZ3}),
one obtains beta functionals for $v_k, V_{F,k}$ and $g_{k',k}$,
\begin{align}
    \FR{\di v_k(\ell)}{\di\ell}    
&= v_k(\ell) 
\Biggl[ 
        -\FR{4(N_c^2-1)}{\pi^3N_cN_f}\FR{g_k(\ell)^2}{V_{F,k}(\ell)}\log\PFR{V_{F,k}(\ell)}{c(\ell)}\Theta_1(\ell,\elltwokf) 
\nn &\hspace{2.0cm}
        - \FR{2(N_c^2-1)}{\pi^4N_c^2N_f^2}
        \FR{g_k(\ell)^4}{c(\ell)^2V_{F,k}(\ell)^2}
            \log^2\PFR{V_{F,k}(\ell)v_k(\ell)}{c(\ell)}
%        \log^2\PFR{V_{F,k}(\ell)c(\ell)}{v_k(\ell)}
        \Theta_1(\ell,\ellonekf) 
\Biggr], 
\label{betaVgen1}\\
%
\FR{\di V_{F,k}(\ell)}{\di\ell}  &= V_{F,k}(\ell)
\Biggl[ 
        \FR{2(N_c^2-1)}{\pi^3N_cN_f}\FR{g_k(\ell)^2}{V_{F,k}(\ell)}\log\PFR{V_{F,k}(\ell)}{c(\ell)}\Theta_1(\ell,\elltwokf)
%\nn &\hspace{2.0cm}
        -\FR{N_c^2-1}{\pi^2N_cN_f}\FR{g_k(\ell)^2}{c(\ell)V_{F,k}(\ell)}\Theta_1(\ell, \elltwokf)
\nn &\hspace{2.0cm}
        -\FR{N_c^2-1}{\pi^2N_cN_f}v_0(\ell)\log\PFR{1}{c(\ell)}
        %-\FR{N_c^2-1}{8\pi^2N_c^2N_f^2}w^2\log^2\PFR{1}{w}
        +\FR{N_c^2-1}{2\pi N_cN_F}w_0(\ell)
\Biggr], 
\label{betaVfgen1}\\
%%
%%
%%
\FR{\di g_{k',k}(\ell)}{\di\ell} &= g_{k',k}(\ell)
\Biggl[ 
        -\FR{1}{2\pi N_cN_f}w_0(\ell)\log\PFR{1}{w_0(\ell)}
        +\FR{N_c^2-1}{2\pi N_cN_f}w_0(\ell)
\nn &\hspace{2.0cm}
        -\FR{N_c^2-1}{\pi^2N_cN_f}v_0(\ell)\log\PFR{1}{c(\ell)} 
        -\FR{N_c^2-1}{8\pi^2N_c^2N_f^2}w_0(\ell)^2\log^2\PFR{1}{w_0(\ell)} 
\nn &\hspace{2.0cm}
        -\FR{(N_c^2-1)g_k(\ell)^2  \Theta_1(\ell, \elltwokf) }{2\pi^2N_cN_fc(\ell)V_{F,k}(\ell) }
        -\FR{(N_c^2-1)g_{k'}(\ell)^2 \Theta_1(\ell, \elltwokpf) }{2\pi^2N_cN_fc(\ell)V_{F,k'}(\ell)}
\nn &\hspace{2.0cm}
        +\FR{g_k(\ell)g_{k'}(\ell)}{2\pi^2c(\ell)N_cN_f}
        \log\PFR{2c(\ell)}{V_{F,k}(\ell)v_k(\ell)+V_{F,k'}(\ell)v_{k'}(\ell)}
        \times
\nn &\hspace{2.0cm}
        \left[\FR{1}{V_{F,k}(\ell)}+\FR{1}{V_{F,k'}(\ell)}\right]
        \Theta_3(\ell, \elltwokf,\elltwokpf,\ellthreekkpf)
%\right.\nonumber\\ &\hspace{0.0cm}\left.  -\FR{(N_c^2-1)}{4\pi^4N_c^2N_f^2}\FR{g_k(\ell)^4}{c(\ell)^2V_{F,k}(\ell)^2}\log^2\PFR{v_k(\ell)}{c(\ell)V_{F,k}(\ell)}\Theta_1(\ellonekf,\ell)
%\right.\nonumber\\ &\hspace{0.0cm}\left.  -\FR{(N_c^2-1)}{4\pi^4N_c^2N_f^2}\FR{g(x',x'; \ell)^4}{c(\ell)^2V_{F,k'}(\ell)^2}\log^2\PFR{v_{k'}(\ell)}{c(\ell)V_{F,k'}(\ell)}\Theta_1(\ellonekpf,\ell)
\nn &\hspace{2.0cm}
        - \FR{N_c^2-1}{4\pi^4N_c^2N_f^2}
        \FR{g_k(\ell)^4}{c(\ell)^2V_{F,k}(\ell)^2}
            \log^2\PFR{V_{F,k}(\ell)v_k(\ell)}{c(\ell)}
        \Theta_1(\ell, \ellonekf) 
\nn &\hspace{2.0cm}
        - \FR{N_c^2-1}{4\pi^4N_c^2N_f^2}
        \FR{g_{k'}(\ell)^4}{c(\ell)^2 V_{F,k'}(\ell)^2}
            \log^2\PFR{V_{F,k'}(\ell)v_{k'}(\ell)}{c(\ell)}
        \Theta_1(\ell, \ellonekpf) 
\Biggr].
\label{mainTextBetaGgen1}
\end{align}
Here  $\ell$ is the logarithmic length scale.
\bqa
\Theta_i( \ell, \ell_1,..,\ell_i) = - \frac{ \partial \log \mathscr{H}_i( \Lambda_f e^{-\ell}, \Lambda_f e^{-\ell_1}, .. , \Lambda_f e^{-\ell_i} )}{\partial \ell}
\eqa
are crossover functions that control 
whether each term in the beta functionals is 
on or off at a given $\ell$.
At short  (long) distance scales with $\ell \ll \min_i\{\ell_i\}$ ($\ell \gg \min_i\{\ell_i\}$),
$\Theta_i( \ell_1,..,\ell_i, \ell) \approx 1$
($\Theta_i( \ell_1,..,\ell_i, \ell) \approx 0$),
and the corresponding term in the beta function is turned on (off).
$\ellonekpf$, $\elltwokpf$ and $\ellthreekkpf$ 
are the logarithmic
length scales that mark three crossovers, 
\begin{align}
        \label{appCross1}   \ellonekf     &= \log \left( \frac{\Lambda_f  }{2 V_{F,k}(\ell) v_k(\ell)k} \right),                           \\ % +\mathfrak{G}(\ell)\\ % - \int_0^\ell \FR{1-z(l)}{z(l)}\dd l, \\
        \label{appCross2}   \elltwokf     &= \log \left( \frac{\Lambda_f  }{2 v_k(\ell) c(\ell)k } \right),                                \\ % +\mathfrak{G}(\ell)\\ %  - \int_0^\ell \FR{1-z(l)}{z(l)}\dd l, \\
        \label{appCross3}   \ellthreekkpf &= \log \left( \frac{\Lambda_f  }{|V_{F,k}(\ell)v_k(\ell)k+V_{F,k'}(\ell)v_{k'}(\ell)k'| } \right). % +\mathfrak{G}(\ell)\\ %  - \int_0^\ell \FR{1-z(l)}{z(l)}\dd l.
%\intertext{where}
%\mathfrak{G}(\ell) &= - \int_0^\ell \FR{1-z(l)}{z(l)}\dd l
\end{align}
%Since \eq{appCross1}-\eq{appCross3} 
%depend on $\ell$ through the scale dependent coupling functions,
These crossover length scales 
are determined from the self-consistent equations, 
\bqa
 \ellonek & = & L^{(2L)}(k; \ellonek), \nn
 \elltwok  & = &  L^{(1L)}(k; \elltwok), \nn
 \ellthreekkp & = & min\{ 
L^{(1L)}(x; \ellthreekkp),
L^{(1L)}(x; \ellthreekkp),  
L^{(1L)}_{k,k'}( \ellthreekkp) 
\}.
\label{SelfConsistentLengthScales}
\eqa
The solutions to the self-consistent equations are 
(see Appendices
\ref{sec:FirstCrossoverScale},
\ref{sec:SecondCrossoverScale},
\ref{sec:ThirdCrossoverScale})
\begin{align}
\ellTwoLoopX & \approx f_0(k) 
%\log\FR{\Lambda_f}{2v_0(0)k}
+\log\FR{\ell_0+f_0(k)}{\ell_0}, \nn
\ellOneLoopX & \approx \ellTwoLoopX +   \log\FR{1}{c(\ellonek)}, \nn
\ellthreekkp & \approx \min(\ell^{(2L)}_{(k+k')/2},\ell^{(1L)}_k,\ell^{(1L)}_{k'}),
\label{eq:crossoverscales}
\end{align}
where $f_0(k)= \log\PFR{\Lambda_f}{2v_0(0)k}$.
%$\ellonek$ ($\elltwok$)
%is the length scale above which the two-loop (one-loop) quantum correction to the fermion kinetic term is turned off.
%For a given $k$, $\ellonek < \elltwok$.
%$\ellthreekkp$ is the length scale above which the one loop Yukawa vertex correction is turned off.

It is useful to define the  energy scales associated with 
$  \elltwok$,
$  \ellonek$,
$  \ellthreekkp$
as
\begin{align}
        \Eonex  \equiv \Lambda_f e^{-\elltwok}, \quad
        \Etwox  \equiv \Lambda_f e^{-\ellonek}, \quad
        \Eonexpx  \equiv \Lambda_f e^{-\ellthreekkp}.
        \label{eq:Etoell}
        \end{align}
%
%
%
%The following momentum dependent crossover scales appear in 
%\eq{eq:allcounterterms},
%\begin{align}
%       \label{appEnCross2} 
%       \Eonex &= 2 v_k c |k|, \\
%       \label{appEnCross1}
%           \Etwox  
%       &= 4 V_{F,k} v_k |k|, \\
%       \label{appEnCross3} 
%       \Eonexpx  &= 
%       \max\left(
%                |V_{F,k} v_k x + V_{F,k'} v_{k'} x' |,
%               2v_k c |k|,
%               2 v_{k'} c |x'| \right).
%\end{align}
$\Eonex$ ($\Etwox $) corresponds to the energy scale below which the one-loop (two-loop) quantum corrections to the fermion self-energy turn off,
and
$\Eonexpx$ is the energy scale below which the one-loop vertex correction turns off.
Physically, each of these  eneregy scales corresponds to 
the minimum that virtual particles within loops carry for given external momenta.
For example, 
consider the self-energy 
diagram for electron.
% with momentum $k$ away from the hot spot. 
%creates a virtual electron and a boson in the one-loop self-energy diagram.
If the external electron is at the hot spot $N$ with $\vec k=0$,
it can be scattered right onto the hot spot $\bar N$ on the Fermi surface 
by emitting or absorbing a boson with momentum $\vec q= 0$.
Since all virtual particles have zero energy,
this gives rise to an infrared divergence in the low-energy limit.
If the external electron is away from the hot spot ($\vec k \neq 0$), 
it is impossible for the electron to be
scattered onto the Fermi surface 
without creating a boson with a non-zero energy.
Inevitably, one has to create a virtual electron away from the Fermi surface
or a virtual boson with a non-zero momentum.
If the virtual electron is on the Fermi surface near hot spot $\bar N$,
the virtual boson has to carry at least momentum $2 v_k k$.
Conversely, if the virtual boson has zero momentum,
the virtual electron has to be away from the Fermi surface with momentum $2v_v k$. 
Since $V_{F,k} \gg c$ in the small $v$ limit, 
it is energetically favorable to create a boson with
 momentum $2 v_k k$ while putting the virtual electron on the Fermi surface.
This gives rise to the infrared energy cutoff $\Eonex = 2 c v_k k$.
%%
%%
For the two-loop self-energy for electron with $k \neq 0$,
unless $v=0$,
it is kinematically impossible to put all virtual electrons
on the Fermi surface 
even at the expense of creating bosons with non-zero energies. 
Since $V_{F,k} \gg c$,
the infrared energy cutoff is determined
by the minimum energy that one of the virtual electron has to carry.
It is order of $V_{F,k} v_k k$.
%%
The expression for $\Eonexpx$ is more complicated
because the vertex correction depends on two external momenta.
When $k+k'=0$, there exists a choice of internal momentum
that puts all virtual electrons on the Fermi surface.
In this case, only boson carries non-zero energy 
and $\Eonexpx$ reduces to 
$\Eonex$.
For $k+k' \neq 0$, the virtual electron is necessarily
kicked away from the Fermi surface due to momentum conservation,
and the infrared energy cutoff is again proportional to 
$V_{F,k} v_k x +V_{F,k'} v_{k'} k'$.
[FIGURES TO BE ADDED]



%\label{EnCross1} \ellonek &= \log \left( \frac{\Lambda_f}{ 2 v(0; \log( \Lambda_f/x)) x} \right), \\ 
%\label{EnCross2} \elltwok &= \log \left( \frac{\Lambda_f}{ 2 v(0;\ellonek) c(\ellonek) x} \right), \\
%\label{EnCross3}  \ellthreekkp &= \min\Bigl(\ell^{(2L)}_{(k+k')/2},\elltwok,\elltwokp\Bigr)
%
%\label{EnCross1} \Etwox &= 
%               \begin{cases}
%               2v_0 x \left(1+\FR{\log\FR{\Lambda_f}{2v_0x }}{\ell_0}\right)
%               & x \gg \Lambda_f e^{-1/\ell_0}
%               \\
%               2\left[\FR{\pi^2 N_c N_f}{2(N_c^2-1)}
%               \FR{1}{\log\FR{\Lambda_f}{x}\log\log\FR{\Lambda_f}{x}}
%               \left( 1+\FR{\ell_0}{\log\FR{\Lambda_f}{x}} \right)
%               \right] x
%               & x \ll \Lambda_f e^{-1/\ell_0}
%               \end{cases},                \\
%\label{EnCross2} \Eonex &=         2 v(0;\ellonek) c(\ellonek) x, \\
%%      \Eonexpx &= \max(E_1((k+k')/2),E_2(k),E_1(k)).
%\label{EnCross3} \Eonexpx &= \max\left( E^{(2L)}((k+k')/2), \Eonex, \Eonexp \right).
%\end{align}





\subsection{Hot, lukewarm and cold electrons}

In this section,
we discuss the solution of the beta functions.
Since the RG flow equations for 
$v_k, V_{F,k}, g_k$ 
do not depend on the off-diagonal 
Yukawa coupling $g_{k',k}$, 
we first solve the beta functions
for  $v_k(\ell), V_{F,k}(\ell), g_k(\ell)$. 
The beta functionals in \eq{mainTextBetaGgen1}
take different forms in each of the three windows of length scale :
(i) $\ell < \ellTwoLoopX$,
(ii) $\ellTwoLoopX < \ell < \ellOneLoopX$,
and (iii) $\ellOneLoopX < \ell$. 
In region i), all quantum corrections are present, and electrons are strongly renormalized 
by spin fluctuations as they are at the hot spots.
In region ii), only one-loop quantum corrections are present 
while the two-loop corrections turned off.
In region iii), all quantum corrections are turned off.
This  is shown in \fig{fig:crossover}.
One first solve the beta functions to obtain
 $J_k^{(i)}(\ell)$, $J_k^{(ii)}(\ell)$, $J_k^{(iii)}(\ell)$ for $J_k=v_k,V_{F,k},g_k$ 
 in each energy window,
 and the coupling functions are matched at the boundary so that they are continuous
 across the crossovers :
 $J_k^{(i)}(\ellTwoLoopX) =J_k^{(ii)}(\ellTwoLoopX)$ 
 and
  $J_k^{(ii)}(\ellOneLoopX) =J_k^{(iii)}(\ellOneLoopX)$.

 
 
For $v \ll 1$,
one can simplify the crossover structure 
by taking advantage of the fact that
all beta functions are small : 
$ \frac{1}{J} \frac{\partial J}{\partial \ell} \sim w \ll 1$
for all couplings.
%, $J = v, V_F, g$.
Since $\ellOneLoopX - \ellTwoLoopX \sim \log 1/c$,
the change of the couplings in region (ii) 
is only 
$\frac{ | J(\ellOneLoopX) - J(\ellTwoLoopX)|}{J(\ellTwoLoopX)} \sim w \log(1/c) \ll 1$ in the small $v$ limit. 
The details can be found in Sec. \ref{sec:SecondCrossoverScale}.
Therefore the flow of all couplings
can be ignored
 in $\ellTwoLoopX < \ell < \ellOneLoopX$,
and one can merge the two crossovers into one.
Therefore, we use  
$J^{(iii)}_k$ in both regions ii) and iii).









%
%
%It is easier to understand the solution for $V_{F,k}(\ell)$ and $g_k(\ell)$ first.
At a given length scale $\ell$,
the Fermi surface can be 
divided into three regions 
divided by $k_h(\ell)$ and $k_c(\ell)$ that satisfy
\begin{align}
\label{defnX1X2}
\ell^{(2L)}_{k_h(\ell)} = \ell, \quad
\ell^{(2L)}_{k_c(\ell)} = 0.
\end{align}
The hot region is given by 
$0 \le |k| \le k_h(\ell)$.
%\frac{ \Lambda_f e^{-\ell}}{2v_0 c(0)}$.
In this region, the momentum  dependent IR cutoff energy scales
are smaller than the energy scale ($\Lambda_f e^{-\ell}$),
and electrons remains strongly coupled with spin fluctuations.
In the hot region,
$v_k$, $V_{F,k}$ and $g_k$ 
flow in the same way as in the hot spots : 
$v_0(\ell)  =   
\FR{\pi^2 N_c N_f}{2(N_c^2-1)}  \FR{1}{(\ell+\ell_0)\log(\ell+\ell_0)}$,
$V_{F,k}(\ell)=1$
and
$g_k(\ell)=\sqrt{\frac{\pi v_0(\ell) }{2}}$ as in  \eq{eq:ZeroMomParam}.
Here $V_{F,k}(\ell)=1$ is the reference speed
which we choose to set to be $1$.
%All speeds are understood to be measured in the unit of the speed of electrons at the hot spots.
%%
%%
The next is the `lukewarm' region given by
 $k_h(\ell)  \le |k| \le  k_c(\ell)$.
 In this region,
the momentum dependent IR cutoff energy scale
is larger than the energy scale
but smaller than the UV cut off, $\Lambda_f$.
Electrons in this range of momentum receive quantum corrections 
within a window of energy scale given by $  \Lambda^f e^{ -\ellonek } < E < \Lambda_f$
before they decouple below $ \Lambda^f e^{ -\ellonek }$.
Once electrons are decoupled,
the coupling with spin fluctuations  
decreases with increasing $\ell$.
In the low energy limit,
$v_k(\ell)$ freezes out.
Furthermore,
spin fluctuations no longer slow electrons down,
and $V_{F,k}(\ell)$ increases
as the Fermi velocity in this range of momentum
 becomes bigger than that of the hot spots.
The momentum profiles of the coupling functions
are determined from the the momentum dependent IR cutoff
which  increases with increasing $k$.
Since electrons farther away from the hot spots 
decouple from spin fluctuations at higher energies,
$g_k(\ell)$ decays while
$v_k(\ell)$ and $V_{F,k}(\ell)$ 
increases with increasing momentum 
at a fixed $\ell$.
%We call this region lukewarm region.
%%
It is noted that the division of 
the hot and lukewarm regions depends
on the energy scale.
As the energy is lowered,
the hot region shrinks
while the lukewarm region grows
as more electrons on the Fermi surface
get decoupled from spin fluctuations
at lower energies.
%%
Finally, electrons with momentum 
$|k| \ge  k_c(\ell)$
are too far away from the hot spots
to receive any significant renormalization
from spin fluctuations 
at any energy below $\Lambda_f$.
In this region, $v_k$ is not renormalized at all,
while $g_k(\ell)$ ($V_{F,k}(\ell)$)  decreases (increases) with increasing $\ell$.
We call this the cold region.


%The crossovers of $v_k(\ell)$ is a bit more complicated
%because both the one-loop and two-loop corrections
%are equally important for the flow of $v$.
%Both quantum corrections make $v$ to decreases at low energies.
%However, the RG speed at which $v$ decreases slows down as the energy is lowered
%as the two-loop correction first  turns off
%below $\Lambda_f e^{-\ellonek}$,
%and the one-loop correction turns off 
%below the lower energy scale, $ \Lambda_f e^{-\elltwok}$.   
%Once both quantum corrections are turned off,
%$v$ saturates to a momentum dependent value in the low-energy limit.
%%
%Due to the presence of the two-loop correction,
%each of the hot and the lukewarm regions 
%is further divided into two subregions
%depending on whether the two-loop quantum corrections
%are on or off.
%In the hot region I with 
%$ 0 \le |k| \le k_h(\ell)$,
%both the one-loop and the two-loop corrections 
%persist down to the energy scale $\Lambda_f e^{-\ell}$,
%and the flow of $v_k(\ell)$ is given by the flow at the hot spot
%upto that energy scale.
%In the hot region II with 
%$k_h(\ell) \le |k| \le k_h(\ell)'$
%with $\ell^{(1L)}_{x_1'} = \ell$,
%the one-loop correction remains turned on upto the energy scale 
%$\Lambda_f e^{-\ell}$,
%but  the two-loop correction is turned off below energy scale  $\Lambda_f e^{-\ellonek}$. 
%Since the two-loop correction turns off at higher energy scales
%for electrons farther away from the hot spots, 
%$v_k(\ell)$ increases with increasing $k$.
%The lukewarm region I is given by
%$k_h(\ell)' \le |k| k_c(\ell)$.
%In this region, electrons receive both one-loop and two-loop quantum correction
%at high energies, but both of them are turned off 
%at energy scales higher than  $\Lambda_f e^{-\ell}$.
%This gives rise to a faster increase of $v_k(\ell)$ as a function of $k$.
%In the lukewarm region II given by
%$k_c(\ell) \le |k| \le k_c(\ell)'$
%with $\ell^{(1L)}_{k_c(\ell)'} = 0$,
%electrons do not experience the two-loop correction
%in any energy scale below the UV cutoff,
%and  receive only the one-loop quantum correction
%in $\Lambda_f e^{-\elltwok} < \mu < \Lambda_f$.
%In the cold region  given by $ \frac{ \Lambda_f}{2v_0 c(0) } \le |k|$,
%electrons do not have any quantum correction
%and the slope of the Fermi surface is not renormalized at all.

%   \vspace{1cm}
%
%   \noindent \emph{TODO} Include figure $E$ vs $k$ and with the high energy,
%   intermediate energy, and low energy regions and show what happens when $\mu \ll
%   \Lambda_fe^{-\ell_0}$.
%
%   \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=1]{./Figures/DiagonalEnergyMomentumCrossoverScalesHighEnergy.pdf}
%   \end{figure}




\begin{figure}[ht!]
        \centering
        \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[scale=.15]{./Figures/figVPLOT.jpg}
        \caption{$v_k(\ell)$ for $\ell = 1,2,3$}
        \label{figVPLOT1}
        \end{subfigure}
 \hspace{1.5cm}
        %
        \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[scale=.15 ]{./Figures/figVFPLOT.jpg}
        \caption{$V_{F,k}(\ell)$ for $\ell = 1,2,3$}
        \label{figVFPLOT2}
        \end{subfigure}
        %
        \\
        %
        \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[scale=.15]{./Figures/figGPLOT.jpg}
        \caption{Diagonal Yukawa coupling $g_k(\ell)$ for $\ell = 1,2,3$}
        \label{figGPLOT1}
        \end{subfigure}
         \hspace{1.5cm}
         %
        \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[scale=0.575]{./Figures/fig4.pdf}
        \caption{Off diagonal Yukawa Coupling}
        % $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
        \label{figGKKP1}
        \end{subfigure}
        \caption{$\Lambda_f = 10$, $v_0(0) = 0.1$}
                \label{fig:vVFg}
\end{figure}




At a given scale $\ell$,
the momentum dependent coupling functions are given by
\begin{align}
\label{vMPsimplified}
v_k(\ell) &= 
\begin{cases}
v_0(\ell)                           & k < k_h(\ell)\\
v_0(\ellonek)                       & k_h(\ell) < k < k_c(\ell)\\
v_0(0)                              &  k_c(\ell) < k
\end{cases}
\\
\label{vfMPsimplified}
V_{F,k}(\ell) &= 
\begin{cases}
1     & k < k_h(\ell)\\
\mc E_1(\ell;\ellonek)              & k_h(\ell) < k < k_c(\ell)\\
\mc E_1(\ell;0)                     &  k_c(\ell) < k
\end{cases}
\\
\label{gxxMPsimplified}
g_k(\ell) &= 
\begin{cases}
\sqrt{\pi v_0(\ell)/2}                             & k < k_h(\ell)\\
\sqrt{\FR{\pi}{2} v_0(\ellonek)} ~ \mc E_0(\ell;\ellonek) & k_h(\ell) < k < k_c(\ell)\\
\sqrt{\pi v_0(0)/2}  ~
\mc E_0(\ell;0)               &  k_c(\ell) < k
\end{cases},
\end{align}
where
\begin{align}
v_0(\ell)  &=   \FR{\pi^2 N_c N_f}{2(N_c^2-1)}  \FR{1}{(\ell+\ell_0)\log(\ell+\ell_0)}, \\ 
\mc E_0(X,Y) &\equiv \exp\left(-\FR{\sqrt{X+\ell_0}-\sqrt{Y+\ell_0}}{\sqrt{N_c^2-1}}\right),\\
\mc E_1(X,Y) &\equiv
\exp\left(\sqrt{N_c^2-1}\left(\mathrm{Ei}(\log\sqrt{X+\ell_0})-\mathrm{Ei}(\log\sqrt{Y+\ell_0})\right)\right).
\end{align}
In \fig{fig:vVFg},
 the momentum profile of the couplings are shown.



Now we turn to the general Yukawa coupling.
%Because $g_{k',k}$ is symmetric under the interchange of $k$ and $k'$,
%we assume  $|k| \ge |x'|$ without loss of generality.
The solution of the beta functional is given by
%In this case, $g_{k',k}(\ell)$ is given by
\begin{align}
\label{eq:gofffinal}
g_{k,k'}(\ell) &= 
\begin{cases}
\sqrt{\FR{\pi}{2}v_0(\ell)}                                   & \ell \le \ellthreekkp\\
\sqrt{\FR{\pi}{2}v_0(\ellthreekkp)}\mc E_0(\ell,\ellthreekkp) & \ell \ge \ellthreekkp.
\end{cases}
\end{align}
%
%\begin{align}
%& g(x',x; \ell) = \nn
%       &
%       \begin{cases}
%   %\left\{
%   %\begin{aligned}
%v_0(\ell) 
%       & \ell \le \ellthreekkp\\
%v_0(\ellthreekkp) \mc E_0( \ell, \ellthreekkp) 
%       & \ellthreekkp \le \ell \le \elltwok\\
%v_0(\ellthreekkp) \mc E_0( \elltwok, \ellthreekkp) 
% \mc E_0( \ell, \elltwok) 
% \sqrt{ \mc E_1( \ell, \elltwok)  } 
%       & \elltwok \le \ell \le \elltwokp\\
%v_0(\ellthreekkp) \mc E_0( \elltwok, \ellthreekkp) 
% \mc E_0( \elltwokp, \elltwok) 
% \sqrt{ \mc E_1( \elltwokp, \elltwok)  } 
% \mc E_0( \ell, \elltwokp) 
% \mc E_1( \ell, \elltwokp)  
%       & \ell \ge \elltwokp
%   \end{cases}.
%       \label{eq:gofffinal}
%\end{align}
\eq{eq:gofffinal}
can be understood in the following way.
The RG flow of $g_{k',k}$ is  
controlled by the vertex correction 
%($A^{(4)}$) 
and the self-energy corrections
%  ($A^{(1)}$) 
to the electrons at momenta $k$ and $k'$.
However, the vertex correction is the dominant factor, and the momentum dependence of the renormalized Yukawa coupling is largely determined by the crossover scale at which the vertex correction turns off.
The vertex correction  tends to enhance the Yukawa coupling.
This anti-screening effect originates from 
the non-Abelian nature of the $SU(N_c)$ group.
At short distance with
$\ell < \ellthreekkp$,
the vertex correction is balanced with
the field renormalization of the boson,
and the Yukawa coupling remains 
order of $\sqrt{v_0}$.
At larger distance scale with $\ell > \ellthreekkp$,
the correction for $g_{k',k}$ turns off.
Because the critical boson still receive field renormalization 
from electrons close to the hot spots,
the decoupling leads to a rapid decay of the Yukawa coupling 
between electrons at non-zero momenta and the boson 
at low energies
as is shown in \eq{eq:gofffinal}.




% 
%Third, the self-energy correction, 
%which makes electrons incoherent,
%has the screening effect that suppresses the Yukawa coupling.
%%%
%%%
%For  $|x'| < |k|$, 
%the momentum dependent infrared cutoffs have the following hierarchy : 
%$\Lambda_f e^{-\ellthreekkp}  >  \Lambda_f e^{-\elltwok} >  \Lambda_f e^{-\elltwokp}$.
%As the energy is lowered.
%the quantum corrections turn off in the order of 
%the vertex correction,
%the self-energy correction at momentum $k$,
%and 
%the self-energy correction at momentum $k'$.
%%%
%In the high energy region in which the energy scale is much larger than
%all momentum dependent infrared cutoff scales,
%the Yukawa coupling flows in the same way as the coupling
%at the hot spot.
%The coupling decays logarithmically following the logarithmic flow of $v_0(\ell) $
%at the hot spots.
%%
%%
%In the lower energy window given by
%$  \Lambda_f e^{-\elltwok} < \mu <  \Lambda_f e^{-\ellthreekkp}$,  
%%$\ellthreekkp \le \ell \le \elltwok$,
%the Yukawa coupling decays at a faster rate.
%This is attributed to the fact 
%the vertex correction drops below  $\Lambda_f e^{-\ellthreekkp}$.
%The disappearance of the anti-screening effect 
%makes $g_{k',k}(\ell)$ to decreases exponentially in $\sqrt{\ell + \ell_0}$.
%As the energy is further lowered, 
%the self-energy correction  also turns off at momentum $k$ 
%below  $ \Lambda_f e^{-\elltwok} $.
%The self-energy correction at momentum $k'$
%turns off  below the lowest IR cutoff scale, $  \Lambda_f e^{-\elltwokp}$.
%The disappearance of the screening effect associated with the
%self-energy corrections slows down the decreases of the Yukawa coupling.
%However, the vertex correction ($A^{(4)}$) is larger than the self-energy correction ($A^{(1)}$) 
%by a factor of $\log c/v$ in magnitude, 
%%as is shown in  Eqs. (\ref{eq:A1}) and  (\ref{eq:A4}),
%and the coupling continues to flow to zero in the low-energy limit. 
%%does not reverse the decreasing flow of the coupling in the low-energy limit.
%
%










%%%%%%%%%%

\subsection{Spectral function}
\label{Sec:Spectral}





In this section, we examine how the electron spectral function varies 
as a function of momentum along the Fermi surface.
The spectral function 
%defined by
%$\mc A(\omega,k_N) = \frac{1}{\pi} \mathrm{Im} G_{\mathrm{R}}(\omega,k_N)$
gives the probability that  
an electron with momentum $\vec k$ 
has energy $\omega$.
Away from the hot spots,
electrons are decoupled from gapless spin fluctuations 
below the momentum dependent crossover scale,
and the spectral function supports 
a sharp quasiparticle peak 
in the low-energy limit. 
Since electrons at different locations 
on the Fermi surface decouple from spin fluctuations at different energy scales,
the quasiparticle weight, Fermi velocity and the shape of Fermi surface
all receive momentum dependent renormalization. 
The spectral function can be readily obtained from the two-point function in \eq{eq:SolRGEq2Point}.
To be concrete,
we assume that the spectral function takes the form of the free fermion 
with $V_{F,k}=1$ and  $v_k=v_0$
at the UV cutoff energy scale $\Lambda_f$.
Here $\Lambda_f$ is the scale 
below which the field theory description is valid.
In reality, the electrons at frequency scale 
$\Lambda_f$ 
are already dressed by quantum fluctuations between the lattice scale and \Lf.
Nonetheless, those high-energy quantum corrections only introduce 
smooth variations in the electronic properties as a function of momentum.
The high-energy renormalization does not affect the singular part of the momentum profile 
that arises due to the coupling between gapless spin fluctuations and electrons
near the hot spots. 
Our goal is to capture the singular profiles of electronic properties 
that are independent of the microscopic details.
%
Setting $\ell$ to $\lo$ 
where $k_0(\lo) = \Lambda_f$
in \eq{eq:ScalingTransfo},
the spectral function is obtained to be  
(see Appendix \ref{chap:2PFELE} for derivation)
\begin{align}
\mc A \left(
\omega,\vec k
\right) 
&= \FR{1}{\pi}
\FR{\mfZ(\omega,k_N) \gamma(\omega,k_N)}{
\Big\{
-\omega+\mfVF(\omega,k_N)e_N[\vec k;v_{k_N}(\mathrm{Re}(\lo))]
\Big\}^2 
+ \gamma(\omega,k_N)^2},
\label{eq:defnSpecFcn}
\end{align}
where
the quasiparticle weight,
the renormalized Fermi velocity
and the quasiparticle decay rate
are given by
%\textcolor{red}{
\begin{align}
\mfZ(\omega,k_N) = \mfVF(\omega,k_N) &= \frac{1}{\mc E_1\left( \min(\mathrm{Re}(\lo),\elltwokN),0 \right)}, \\
%\mfVF(\omega,k_N) &= \frac{1}{\mc E_1\left( \min(\mathrm{Re}(\lo),\elltwokN),0 \right)}, \\
\label{mcT}
\gamma(\omega,k_N) &=
\begin{cases}
%
-\FR{\pi \omega\sqrt{N_c^2-1}}{4\sqrt{\mathrm{Re}(\lo)+\ell_0}\log\sqrt{\elltwokN+\ell_0}}
-\FR{\pi  v_0( \mathrm{Re}(\lo)) k_N  \mc E_1(\mathrm{Re}(\lo),0)^{-1}}{2(\mathrm{Re}(\lo)+\ell_0)} 
%
& \mathrm{Re}(\lo) \ll \elltwokN
%\elltwokN\ll\elltwokN
\\
-\FR{\pi\omega\sqrt{N_c^2-1}}{2\sqrt{
\elltwokN
+\ell_0}\log(\elltwokN+\ell_0)}
\FR{\exp(-\mathrm{Re}(\lo))}{\exp(-\elltwokN)}
\FR{\exp(-\sqrt{\mathrm{Re}(\lo)+\ell_0}/\sqrt{N_c^2-1})}{\exp(-\sqrt{\elltwokN+\ell_0}/\sqrt{N_c^2-1})}
&\mathrm{Re}(\lo)\gg\elltwokN,
\end{cases}
%\label{eq:ZVFgamma}
\end{align}
where
\begin{align}
\label{eq:ellomega}
\lo 
%&= \log\FR{\Lambda_f}{-i\omega} - \FR{ \sqrt{N_c^2-1}\sqrt{ \ell_0 + \log\FR{\Lambda_f}{-i\omega} } }{ \log\sqrt{\ell_0 + \log\FR{\Lambda_f}{-i\omega}} } + \FR{ \sqrt{N_c^2-1}\sqrt{ \ell_0 } }{ \log\sqrt{\ell_0} } \nn
&= \left[
 \log\FR{\Lambda_f}{\omega} - \FR{ \sqrt{N_c^2-1}\sqrt{ \ell_0 + \log\FR{\Lambda_f}{\omega} } }{ \log\sqrt{\ell_0 + \log\FR{\Lambda_f}{\omega}} } + \FR{ \sqrt{N_c^2-1}\sqrt{ \ell_0 } }{ \log\sqrt{\ell_0} }
 \right]
+  i \FR{\pi}{2}.
\end{align}
We note that 
$\mfVF(\omega,k)$ is different from $V_{F,k}$.
The former is the actual Fermi velocity of an electron at
momentum $k$ away from the hot spots,
whereas the latter is the ratio between the Fermi velocity at momentum $k$
and the Fermi velocity at the hot spots.

\begin{figure}
    \centering 
    \includegraphics[scale=0.3]{./Figures/NFL2FLcrossover.pdf}
    \caption{
         {\bf[ Updated August 1, 2020. ]}
         This is the crossover scale at low-energies.
         \com{
         1) Relabel the region : 'Crossover' into 'NLFL' (non-Landau FL)
         2) add equations for each curve
         3) change colors to deliver intuitive picture
                         : NFL (orange; hotter), 
                         Non-Landau LF (green; warm),
                     FL ( blue; cold)
         }
    } 
\label{fig:crossoverNFLtoFL}
\end{figure}
 
 
 
To the leading order in $v$,
$\mfZ(k_N) = \mfVF(k_N)$ because
both the quasiparticle weight and the Fermi velocity
are determined by the frequency dependent self-energy correction, $Z^{(1)}(k)$
that renormalizes both the electron field and the Fermi velocity.  
$\mfZ(k_N) = \mfVF(k_N) =1$
at momenta far away from the hot spots with 
$k_N > k_c(\ell)$
because 
electrons in the cold region 
are not renormalized.
Electrons with $k_h(\ell) < k < k_c(\ell)$ are subject to 
renormalization caused by spin fluctuations at energies lower than \Lf
but eventually decouple from spin fluctuations 
below energy scale $\Lambda_f e^{-\ellTwoLoopX}$.
%  that is proportional to the displacement
%from the hot spots in the momentum space.
%For $Z^{(1)}(k)$, this decoupling happens at $\Lambda_f e^{-\elltwok}$.
Since electrons closer to the hot spots remain coupled with spin fluctuations over longer length scales,
the quasiparticle weight and the Fermi velocity decreases as momentum approaches 
the hot spots on the Fermi surface. 
%in which the flow of $v$ can be ignored.
%In this case, $\mfZ(k_N)$ and $\mfVF(k_N)$ decays as a power-law
%in the momentum along the Fermi surface with the exponent  that is proportional to
%$\frac{v(0,0)}{c(0)} \sim  \sqrt{\FR{N_c^2-1}{\ell_0}}$.
For momenta closer to the hot spots with $k_N < k_h(\ell) $,
the coupling to the spin fluctuations persists down to 
 the energy scale at which the spectral function is probed.
As a result, the quasiparticle weight vanishes in the zero-energy limit at the hot spots.



For 
$\lo \ll \elltwokN$,
%there are two contribution to the imaginary part of the self-energy.
%The first term arises from the scale dependence 
%of $F_z$ while the second term is from 
%$v_{k_N}(\ell)$.
%%
%%
%In this high energy region,
the decay rate is linear in energy up to logarithmic corrections.
%The line width is is barely smaller than the quasiparticle energies.
This non-Fermi liquid behaviour persists 
down to zero-energy limit at the hot spots.
Away from the hot spots, 
the  $\omega$-linear decay rate at high frequency crossovers
to a decay rate that goes as $\omega^2$ 
at energies below the crossover scale.
Therefore, quasiparticles are well defined 
in the low-energy limit away from the hot spots.
%Away from the hot spots, low-energy electronic excitations are 
%well described by quasiparticles.
These two distinct behaviours are continuously connected in the momentum space
as the quasiparticle weight continuously decays to zero 
as the hot spots are approached along the Fermi surface.
%
In the non-Fermi liquid (NFL) region with $\omega > 2 v_0 c(0) k_N$,
the critical spin fluctuations destroy coherence of quasiparticle.
In the Fermi liquid (FL) region with $\omega < 2 v_0 c(0) k_N$,
the quasiparticles are well defined.

%
%
%
%In Fermi liquids in two dimensions, 
%the scattering by short-range four-fermion interactions
%gives rise to the line width that goes as 
%$\mc T_{FL} \sim \omega^2\log(1/\omega)$ in the low-frequency limit.
%At sufficiently low energies below a new crossover energy scale given by
%\begin{align}
%       \omega_{\textrm{crossover}}(k) &= \exp\left(-\left[\log\FR{\Lambda_f}{2vck}\right]^2\right), 
%\end{align}
%the contribution from the short-range four-fermion coupling dominates
%the line width. 
%Above the new crossover scale, 
%the line width due to the critical spin fluctuations.
%This gives rise to three regions in the plane of frequency and momentum along the Fermi surface
%as is shown in 
%\fig{fig:crossoverNFLtoFL}.
%In the non-Fermi liquid (NFL) region with $\omega > 2 v_0 c(0) k_N$,
%the critical spin fluctuations destroy coherence of quasiparticle.
%In the Fermi liquid (FL) region with $\omega <    \omega_{\textrm{crossover}}(k) $,
%the short-range four-fermion coupling dominates the decay rate of single-particle excitations.
%In the intermediate region between NFL and FL regions, 
%the quasiparticles are well defined but
%the decay rate is larger than 
%that of the standard Fermi liquids.
%This intermediate region is called non-Landau Fermi liquid (NLFL) region. 






% and scales as  $\omega^2\exp(-\sqrt{\log(1/\omega)+ \ell_0})$.

% with an additional momentum-dependent prefactor. 
%In the low-$\omega$
%limit we see that the scattering by effective four-fermion interactions is
%dominant over the scattering from the collective mode. 
%%
%However, at the hot spot the scattering rate due to the collective mode is
%linear in $\omega$ and thus in the low-energy limit it is this scattering
%channel that dominates, cf. eqn.~(\ref{eq:SpectralHotspots}). 
%%
%Because there is a continuous transition, we should expect that the
%linear-in-$\omega$ dependence will dominate the $\omega^2$ dependence in a
%region near the hot spot. 


%Let us fix a non-zero frequency $\omega$ and additionally assume that $\omega
%\gg \omega^2$ and ask at what momentum does the decay rate due to the collective
%mode, $\mcTnfl(\omega,k_N)$, equal the Fermi liquid decay rate, $\mcTfl(\omega)
%\sim \omega^2\log(1/\omega)$. In the low energy limit for $\lo \gg \ell_0$ we
%get:





%\bqa
%\mc T(\omega,k_N) 
%&=& 
% \begin{cases}
%% \frac{\omega\,\mathrm{Im}\left[\mc F_z^{(1)}(\omega,k_N)\right]}{\mc F_z^{(0)}(k_N)}
%       \FR{\omega^2}{2vck_N}
%       \FR{\sqrt{N_c^2-1}}{\sqrt{\elltwokN+\ell_0}\log(\elltwokN+\ell_0)} 
%       \FR {(\lo+\ell_0)^{3/2}\exp\left(-\nu_1\sqrt{\lo+\ell_0}\right)}
%           {(\elltwokN+\ell_0)^{3/2}\exp\left(-\nu_1\sqrt{\elltwokN+\ell_0}\right)},
%           &\omega /2v_0 c(0) < k_N  \\
%\omega \left(\frac{ \pi  \sqrt{N^2-1} \left(\log \left(\sqrt{\log
%   \left(\frac{\Lambda }{\omega }\right)+l_0}\right)-1\right)}{4 \log ^2\left(\sqrt{\log
%   \left(\frac{\Lambda }{\omega }\right)+l_0}\right) \sqrt{\log \left(\frac{\Lambda
%   }{\omega }\right)+l_0}}\right),
%               &\omega /2v_0 c(0) > k_N 
%   \end{cases}
%\eqa
%\com{Double check the above expression and include derivation in the appendix}




%\begin{figure*}
%   \centering 
%   \includegraphics[scale=0.58,trim={2cm 0 0 0}]{./Figures/qpw_NOSC.pdf}~~
%   \includegraphics[scale=0.58]{./Figures/qpw_NOSC_log.pdf}
%   \caption{
%   \bf{[ Revise the figure]}
%   Momentum profile of the quasiparticle weight and renormalized Fermi velocity. The plot in the right panel is in logarithmic scale.
%       }
%        \label{fig:qpwnosc}
%\end{figure*}


%\begin{figure*}
%   \centering 
%   \includegraphics[scale=0.58,trim={2cm 0 0 0}]{./Figures/qpwLinearLinearUPD1.pdf}~~
%   \includegraphics[scale=0.58]{./Figures/qpwLogLogUPD1.pdf}
%   \caption{
%         {\bf[ Updated July 3, 2020. ]}
%         Momentum profile of the quasiparticle weight and renormalized Fermi
%         velocity. The plot in the right panel is in logarithmic scale.
%    }
%    \label{fig:qpwnosc}
%%\label{fig:qpwupd1}
%\end{figure*}
%


%an energy scale
%in which the flow of $v$ is no longer negligible.
%In that low-energy regime, $\frac{v(0,\ell)}{c(\ell)}$ that flows to zero as $\ell^{-1/2}$  
%gives rise to a decay of  $\mfZ(k_N)$ and $\mfVF(k_N)$.
%This decay is slower than power-law in momentum but
%faster than any finite power of logarithm
%as is shown in the last line of \eq{eq:specZVF}.
%We refer to this as super-logarithmic decay.
%The full momentum profile of    $\mfZ(k_N)$ and $\mfVF(k_N)$ is shown in \fig{figRENORMVF}.

 
 
 
\begin{figure}[ht!]
\centering
\includegraphics[scale=.2]{./Figures/figRENORMVF.jpg}
\caption{Renormalized Fermi Velocity $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
%\includegraphics[scale=.2]{./Figures/fig5.jpg}
%\caption{Off diagonal Yukawa Coupling $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
\label{figRENORMVF}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[scale=.2]{./Figures/figQUASIPARTWEIGHT.jpg}
\caption{Quasiparticle Weight $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
%\includegraphics[scale=.2]{./Figures/fig6.jpg}
%\caption{Off diagonal Yukawa Coupling $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
\label{figQUASIPARTWEIGHT}
\end{figure}
{\ }

\newpage

{\ }
\begin{figure}[ht!]
\centering
\includegraphics[scale=.2]{./Figures/figLIFETIME.jpg}
\caption{
Quasiparticle decay rate with $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$
{\bf changed from lifetime }
}
%\includegraphics[scale=.2]{./Figures/fig7.jpg}
%\caption{Off diagonal Yukawa Coupling $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
\label{figLIFETIME}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[scale=.2]{./Figures/figRENORMFERMISURFACE.jpg}
\caption{Renormalized Fermi surface near hot hot spot $(k=0)$; $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
%\includegraphics[scale=.2]{./Figures/fig8.jpg}
%\caption{Off diagonal Yukawa Coupling $\Lambda_f = 10, v_0(0) = 0.1, \ell = 4$}
\label{figRENORMFERMISURFACE}
\end{figure}

 \begin{figure*}
    \centering 
    \includegraphics[scale=0.58,trim={2cm 0 0 0}]{./Figures/angle_NOSC.pdf}~~
    \includegraphics[scale=0.58]{./Figures/angle_NOSC_log.pdf}
    \caption{
\bf{[ Revise the figure]}
Momentum profile of the slope along the renormalized FS. The plot in the right panel is in logarithmic scale.
} 
\label{fig:nosc}
\end{figure*}

%
%\begin{figure*}
%   \centering 
%   \includegraphics[scale=0.58,trim={2cm 0 0 0}]{./Figures/angleLinearLinearUPD1.pdf}~~
%   \includegraphics[scale=0.58]{./Figures/angleLogLinearUPD1.pdf}
%   \caption{
%         {\bf[ Updated July 3, 2020. ]}
%         Momentum profile of the slope along the renormalized FS. The plot in the right
%         panel is in log-linear
%        %logarithmic 
%        scale.
%    } 
%%\label{fig:angleupd1}
%\label{fig:nosc}
%\end{figure*}
%

The momentum profile of $v_{k_N}$ 
in \eq{vMPsimplified} can be understood 
in a similar manner.
%There are more crossovers for $\vle(k_N)$ 
%because the shape of the Fermi surface is renormalized both by the one-loop and the two-loop
%self-energy corrections to the leading order in $v$, 
%and the two quantum corrections decouple at different energy scales.
%The two-loop quantum correction decouples at the energy scale
%($\Lambda_f e^{-\ellonek}$)
%that is higher than the energy scale ($\Lambda_f e^{-\elltwok}$) 
%below which the one-loop correction decouples.
For  $k_N > k_c(\ell)$, 
the shape of the Fermi surface is not renormalized and
$v_k(\infty) =v_0$.
Below momentum $k_c(\ell)$,
the angle of the Fermi surface begins to receive quantum corrections.
The quantum correction renormalizes the angle to a smaller value 
as the spin fluctuations drive the patches of the Fermi surface connected by 
$\vec Q_{AF}$ closer nesting.
This causes $v_k(\infty)$ to decays with decreasing  $k$ 
and vanishes at the hot spots.
%with the exponent $1/2 \ell_0$.
The full momentum profile of  $\vle(k_N)$ is shown in \fig{fig:nosc}.
{\bf [  the plots for $v_k(\infty)$ to be revised ]}
 


  





